CurvingLoRa to Boost LoRa Network Capacity via Concurrent Transmission

LoRaWAN has emerged as an appealing technology to connect IoT devices but it functions without explicit coordination among transmitters, which can lead to many packet collisions as the network scales. State-of-the-art work proposes various approaches to deal with these collisions, but most functions only in high signal-to-interference ratio (SIR) conditions and thus does not scale to many scenarios where weak receptions are easily buried by stronger receptions from nearby transmitters. In this paper, we take a fresh look at LoRa's physical layer, revealing that its underlying linear chirp modulation fundamentally limits the capacity and scalability of concurrentLoRa transmissions. We show that by replacing linear chirps with their non-linear counterparts, we can boost the capacity of concurrent LoRa transmissions and empower the LoRa receiver to successfully receive weak transmissions in the presence of strong colliding signals. Such a non-linear chirp design further enables the receiver to demodulate fully aligned collision symbols - a case where none of the existing approaches can deal with. We implement these ideas in a holistic LoRaWAN stack based on the USRP N210 software-defined radio platform. Our head-to-head comparison with two state-of-the-art research systems and a standard LoRaWAN baseline demonstrates that CurvingLoRa improves the network throughput by 1.6-7.6x while simultaneously sacrificing neither power efficiency nor noise resilience. An open-source dataset and code will be made available before publication.

==> CurvingLoRa NSDI 22/10Conclusion.tex <==
\section{Conclusion}
\label{sec-conclusion}
We have presented the design, implementation, and evaluation of \ours, a PHY-layer amendment to LoRaWAN. By replacing the linear-chirp modulation on standard LoRaWAN with its non-linear chirp counterpart, the receiver can effectively demodulate large numbers of collided LoRa transmissions in extreme SNR, SIR, and symbol offset conditions.
We practice this idea by design a holistic PHY-layer and implement it on software defined radios.
The results demonstrate \ours improves the network throughput by 7.6$\times$ against the standard LoRaWAN, outperforming two state-of-the-art approaches by 1.6$\times$ and 2.8$\times$, respectively.

% In this paper, we present \ours which boosts LoRaWAN capacity by creating more logical channels with nonlinear chirps. First, we develop a unified symbol modulation method which easily explores a nonlinear function to modulate data with different bandwidth and SF settings. Then, for symbol demodulation, we develop a heuristic method to effectively synchronize baseline down-chirp to received shifted up-chirps. The channel throughput of \ours is the same with LoRa under the identical bandwidth and SF setting. Moreover, \ours is resilient to Gaussian environment noise, thus can support long distance communication as LoRa does. We further develop a SIR based interference model to depict the mutual influence between a pair of linear/nonlinear chirps. Our analysis results show that in comparing with LoRa linear chirp, \ours nonlinear chirps are less influenced by self-interference, but SF is less effective to create logical channels, especially with a high-degree polynomial function. Finally, based on our interference model, we develop a greedy algorithm to select a set of linear/nonlinear logic channels which can maximize LoRaWAN capacity. We implement \ours prototype on HackRF and USRP, then conduct extensive experiments to evaluate its performance. The results show that \ours capacity is 6.15 times higher than LoRaWAN capacity only using linear chirps.


==> CurvingLoRa NSDI 22/1abstract.tex <==
\begin{abstract}
\noindent{}LoRaWAN has emerged as an appealing technology to connect IoT devices but it functions without explicit coordination among transmitters, which can lead to many packet collisions as the network scales. State-of-the-art work proposes various approaches to deal with these collisions, but most functions only in high signal-to-interference ratio (SIR) conditions and thus does not scale to many scenarios where weak receptions are easily buried by stronger receptions from nearby transmitters.  In this paper, we take a fresh look at LoRa's physical layer, revealing that its underlying linear chirp modulation fundamentally limits the capacity and scalability of concurrent LoRa transmissions. We show that by replacing linear chirps with their non-linear counterparts, we can boost the capacity of concurrent LoRa transmissions and empower the LoRa receiver to successfully receive weak transmissions in the presence of strong colliding signals. Such a non-linear chirp design further enables the receiver to demodulate fully aligned collision symbols --- a case where none of the existing approaches can deal with.
We implement these ideas in a holistic LoRaWAN stack based on the USRP N210 software-defined radio platform.
Our head-to-head comparison with two state-of-the-art research systems and a standard LoRaWAN baseline demonstrates that \ours improves the network throughput by 1.6--7.6$\times$ while simultaneously sacrificing neither power efficiency nor noise resilience.
An open-source dataset and code will be made available before publication.

%on an anonymous
%Github link: \textcolor{mypink}{\url{https://github.com/xxxxxxxxxx}}

% Long Range Wide Area Network (LoRaWAN), using linear chirp modulation, is known for its low-power and long-distance communication so that can connect various Internet-of-Things devices at low cost.
% For dense and large-scale IoT deployments, however, LoRaWAN throughput is far from needed due to the frequent collisions.
% A signal is easily corrupted by a stronger one under the standard dechirp decoding. 
% Some approaches explore new features to resolve collisions. However, the concurrency requires higher signal-to-noise ratio (SNR) or matched signal-to-interference ratio (SIR) among collided signals, which degrades the communication range and energy efficiency accordingly.
% %
% %In this paper, we propose \ours to surmount the ceiling of LoRaWAN throughput by embracing nonlinear chirps.
% In this paper, we propose \ours, a brand-new low-power and long-range communication primitive by embracing non-linear chirps that enables concurrent transmission with SNR and SIR tolerance.
% %
% We propose an end-to-end coding framework for any polynomial shape chirp, which provides similar noise resilience as linear chirp.
% Due to its non-linearity, a signal becomes decodable even if it is interfered by stronger signals or noises.
% %
% To make it work in practice, we design an adaptive preamble, consisting of both linear and non-linear chirps, to efficiently synchronize symbols.
% %
% Additionally, we design a media access control strategy by setting different spreading factors (SFs) to optimize network throughput according to the interference level.
% %First, we use nonlinear chirps to enlarge the number of logical channels. 
% %Then, we develop a coexistence model to depict the collision constraints among various types of logical channels. 
% %We further select a set of collision-resilient logical channels to achieve the optimal network capacity.
% %
% We implement \ours with USRPs and conduct extensive experiments in our indoor and campus-scale testbeds. 
% The performance evaluations show that network throughput using \ours is ?? times higher than state-of-the-arts.

\end{abstract}



==> CurvingLoRa NSDI 22/2Introduction.tex <==
\section{Introduction}
\label{sec-intro}
% Introduce the background of LPWAN
% In the past decades, Bluetooth Low Power (BLE)~\cite{das2016uncovering, jeon2018ble} and 802.15.4~\cite{greenorbs, citysee} radios have shown their success to build personal and local area networks for the Internet-of-Things (IoT). 
% Nowadays, billions of untethered IoT devices scattered in wide areas (e.g., industry, agriculture, city, logistic) are being connected. A coming challenge is to scale low-power IoT to these wide areas in a low-cost manner. To mitigate this gap, recent years have witnessed Low-Power Wide Area Networks (LPWAN) emerge as an attractive IoT architecture.

As we gradually reach a cyber-physical world where everything near and far is  connected wirelessly, a fundamental question worth discussing is which wireless technologies are best suited for achieving this goal. While Wi-Fi and cellular networks have proved their success in provisioning high-throughput wireless connectivity in small geographic areas, a remaining challenge is connecting those low-power IoT devices deployed in wide areas. Most of these devices are powered by batteries and thus require minimal communication overhead.


LoRaWAN~\cite{alliance2020lorawan} has emerged as a competitive solution because of its ability to communicate over a large distance. Central to LoRaWAN is a dedicated PHY-layer design that leverages Chirp Spread Spectrum (CSS) modulation to facilitate packet decoding in extremely harsh SNR conditions (which can be as low as $-20$~dB \cite{LoSee}). 
Coupling with a long-term duty cycling mechanism, a deployed LoRa node can last for a few years with a single dry-cell battery.
These dual merits of low-power and long-range make LoRaWAN an attractive solution for IoT connectivity outdoors.

Unlike Wi-Fi, which uses {\it carrier sensing}~\cite{cali2000dynamic} to avoid packet collisions, LoRaWAN functions without explicit coordination due to its stringent power budget. It instead adopts the least restrictive MAC protocol---ALOHA~\cite{abramson1970aloha}---that allows participating nodes to transmit immediately once they wake up.\footnote{LoRaWAN recently released a new feature called Channel Activity Detection
(CAD) that allows the receiver to scan the channel before transmitting. CAD however incurs extra power consumption and thus may not be applicable to rural deployments where battery replacement is usually infeasible.} Such {\it laissez-faire} transmission inevitably causes packet collision when multiple LoRa nodes transmit simultaneously, resulting in retransmissions that can drain the battery of collision nodes and crowd the precious wireless spectrum on the unlicensed band. 
Packet collisions are exacerbated with increased network size, thus reducing throughput and hence fundamentally challenging the scalability of LoRa networks in real deployment.



\begin{figure}[t]
    \centering
    \includegraphics[width=3.2in]{./figures/fig_intro.pdf}
    \vspace{-4mm}
    \caption{An illustration of \ours's energy converging and scattering effect. (a): The energy of a non-linear chirp symbol will converge to a specific frequency point when it aligns with the down-chirp. (b): The energy will spread into multiple FFT bins when this non-linear chirp mismatches with the down-chirp.}
    \label{fig:intro}
    \vspace{-4mm}
\end{figure}

% While above ideas have demonstrated their efficacy, they still face two scalability issues that fundamentally challenge their applicability in practice:
% First, the vast majority of these approaches do not scale to a large number of concurrent transmissions. For instance, mLoRa~\cite{mLoRa} and FTrack~\cite{xia2019ftrack} barely support up to three concurrent transmissions to maintain a symbol error rate less than 0.1. While Choir~\cite{eletreby2017empowering} improved over the above methods, it does not scale to more than ten devices. Although NScale~\cite{tong_combating_2020} can support tens of concurrent transmissions, it requires the overlap ratio between different symbols to be lower than a rigid threshold, which is unlikely to be held in practice given laissez-faire LoRa transmissions.
% Second, none of the foregoing approaches scale well to near-far deployment scenarios. This is due to the fact that after dechirping, the weak reception from a remote transmitter produces a tiny FFT peak that is likely to be buried by strong FFT peaks from LoRa nodes that are closer to the receiver. 
% Although successive interference cancellation (SIC) can be leveraged to deal with this near-far issue~\cite{eletreby2017empowering,mLoRa,shahid2021concurrent}, it functions only in high SNR conditions (\S\ref{subsec-background-3}) to ensure the strong transmissions can be recovered and then canceled out. This sacrifices the noise resilience of chirp signals.


\parabreak{}In this paper, we take a fresh look at the physical layer design of LoRaWAN and reveal that the underlying {\it linear chirp based modulation} fundamentally limits the capacity and scalability of concurrent LoRa transmissions.
We present \ours, a simple but effective PHY-layer design to boost the LoRa network capacity by simply replacing the standard linear chirp with its nonlinear chirp counterpart.

\ours is based on a unique property of non-linear chirps, which we term the {\it energy scattering and converging effect}. When a non-linear up-chirp symbol misaligns with the non-linear down-chirp during demodulation, their multiplication will {\it spread} the power of the non-linear up-chirp symbol into multiple FFT bins where the associated energy peaks are inherently weak. 
Such energy scattering effect will show up as long as the non-linear up-chirp is not well aligned with the down-chirp (The theoretical analysis is in Appendix \ref{appendix-2}). 
In contrast, when this non-linear up-chirp is well aligned with the down-chirp, its signal power will {\it converge} to a specific frequency point, leading to a strong energy peak after FFT (shown in Figure~\ref{fig:intro}).

This allows the receiver to manipulate the signal-to-interference ratio (SIR\footnote{Defined as the ratio between the power of the targeted LoRa chirp and the power of remaining concurrent LoRa chirps.}) of each collision symbol for reliable demodulation. 
In contrast, the power of linear chirps will be always {\it converging} to a single frequency point regardless of its alignment with the down-chirp in demodulation process. This energy converging effect fundamentally limits the decodability of linear chirps in the presence of collisions.

We analyze the performance of non-linear chirp and compare it with its linear chirp counterpart in various SNRs, SIRs, and symbol overlapping ratio conditions.
We show that such a non-linear chirp remarkably improve the transmission concurrency while retaining both the high power efficiency and strong noise resilience as linear chirp does (\S\ref{sec-design}).
We then design a holistic PHY-layer to realize non-linear chirp modulation and demodulation (\S\ref{sec-system}) and implement it on software-defined radios for evaluation.
The experimental results show that compared to two state-of-the-art systems~\cite{mLoRa,tong_combating_2020}, \ours can effectively improve the network throughput by $1.6-6.6\times$ and $2.8-7.6\times$ in an indoor and outdoor deployment, respectively. We make following contributions:

\begin{itemize}[leftmargin=*]
    \item We reveal that the PHY-layer design of LoRaWAN fundamentally limits the transmission concurrency and propose a simple but effective solution. Our approach takes the advantage of power scattering effect of non-linear chirps to enable LoRa concurrent transmissions in extreme SNR, SIR, and symbol overlapping ratio conditions.
    \item Through both theoretical analysis and experimental validation, we demonstrate that \ours outperforms both the current practice and the standard LoRaWAN while sacrificing neither the power efficiency nor noise resilience. These desired properties make non-linear chirp a potential complementary solution to its linear chirp counterpart. %We then demonstrate the feasibility of non-linear chirp-based LoRa transmissions with a holistic PHY-layer design.
    \item We design a holistic PHY-layer and implement it on software defined radios platform to evaluate \ours in various real-world scenarios. The results confirm  that the \ours can greatly improve the network throughput.
\end{itemize}

%novel PHY-layer amendment to LoRaWAN that embodies a suit of modulation and demodulation algorithms to boost the concurrency in LoRa transmissions. Our key idea is to replace the standard linear chirp modulation in LoRa with its non-linear counterpart and exploit the resulting energy pattern (after de-chirping at the receiver) associated with the non-linear chirp to accommodate concurrent LoRa transmissions. 
%Similar to prior works~\cite{}, we make an valid assumption that the collision symbols are not strictly aligned due to the lengthy airtime of LoRa packet.
%\textcolor{red}{XXXX}

% To see how non-linear chirp assists concurrent LoRa transmissions, consider the scenario shown in Figure~\ref{}, where multiple transmitters send LoRa packets at the same time. ....

% The rest of paper is organized as follows. We introduce the LoRa primer in  $\S$\ref{sec-background} and analyze the non-linear chirps in $\S$\ref{sec-design}.
% \S\ref{sec-system} presents the PHY-layer realization of non-linear chirps.
% We detail the system implementation and evaluation in $\S$\ref{sec-implementation} and \S\ref{sec-evaluation}, respectively. 
% The related work ($\S$\ref{sec-related-work}) follows. 
% We conclude the paper in $\S$\ref{sec-conclusion}. 


% While the above ideas have demonstrated their effectiveness in various aspects, we found that all these design innovations inevitably bring two issues that fundamentally challenge their applicability in practice.
% $i)$: SNR loss caused by the phase shift in SIC and intra-symbol fragmentation.
% $ii)$: 


%the vast majority of the design innovation has taken place at the receiver end, leaving the underlying PHY-layer modulation (i.e., linear chirp based) unchanged.




%Introduce LoRaWAN
% LoRaWAN~\cite{alliance2020lorawan} is an open network standard, in which LoRa radios directly communicate with LoRa gateways operating on unlicensed spectrum.
% LoRa physical layer leverages Chirp Spread Spectrum (CSS) to achieve long-distance and low-power data transmission. 
% The commercial-off-the-shelf (COTS) LoRa gateway~\cite{SX1255} can successfully demodulate data packet transmitted kilometers away whose signal-to-noise ratio (SNR) is as low as -20 dB~\cite{LoSee}. 
% The COTS LoRa radios~\cite{sx127x} reach the peak power consumption 400 mW when transmitting at 20 dBm, but draw 5 $\mu$W in the idle mode.
% Due to the long-distance, low-power and low-cost characteristics, LoRaWAN becomes a popular LPWAN protocol.

%%-
% raw text
%LoRa throughput challenge and existing solutions
% In the US, the range of LoRaWAN spectrum is from 902.3 MHz to 914.9 MHz, which is further divided to 64 narrow-band (e.g., 125 kHz) physical channels~\cite{lora_survey_1}.
% To further improve the throughput for each physical channel, the Spreading Factors (SFs) defines the number of bits that can be encoded per symbol and can be configured to trade off the channel throughput and SNR requirement of packet reception`\cite{lora_survey_2,lora_survey_3}. Meanwhile, experimental evaluations demonstrate the orthogonality of configurations with various SFs (e.g., from 7 to 12)~\cite{mahmood2018scalability}, enabling simultaneous packets receptions even under the same physical channel.
% In other words, the ceiling of LoRaWAN throughput is bounded by the number of different channels and SFs.
% When connecting a large number of IoT devices for most LoRa applications~\cite{ghena2019challenge,LoSee, citysee, greenorbs}, packet collisions occurs inevitably in LoRa networking since these physical channels with limited configurations of SFs would be fully occupied. And collisions adversely cause packet loss and throughput degradation, which also drain battery life and waste precious air time and spectrum~\cite{colora,tong_combating_2020}. 
% Given the simple MAC layer design for design simplicity and energy conservation (e.g., ALOHA based MAC protocol in LoRaWAN), collisions can be exacerbates in LoRa networks in the case of a star-of-stars topology where thousands of LoRa nodes connect to a single LoRa gateway.
% An urgent and challenging problem is \emph{can we break the ceiling of LoRaWAN throughput, especially in a dense deployment?}  

% \vspace{1mm}
% \noindent
% \textbf{Status Quo and their limitations:}
% A large collection of collision decoding approaches have been proposed to resolve the collision problem, and the main idea is fully understand and explore the coding properties of LoRa and its CSS modulation scheme across time~\cite{mLoRa,oct,xia2019ftrack}, frequency~\cite{colora,tong_combating_2020,xu_fliplora_2020,eletreby2017empowering}, or even multiple domains~\cite{hu2020sclora}. For example, mLoRa~\cite{mLoRa} detects the collision-free packets from the beginning and decode them iteratively via the Successive Interference Cancellation (SIC)~\cite{gollakota2009interference,mollanoori2013uplink}, achieving throughput improvements of 3$\times$ with up to three concurrent transmissions. 
% FTrack~\cite{xia2019ftrack} further jointly exploits the distinct \textit{frequency tracks} with \textit{misaligned edges} of periodical LoRa symbols to separate collisions to boost the throughput of real-world LoRa by up to 3$\times$.
% However, all temporal features of chirp symbols have fundamental limitations in decoding low SNR LoRa signals (e.g., SNR < 0), as they focus on time domain signal analysis and do not consider the CSS mechanism of LoRa~\cite{colora,tong_combating_2020,xu_fliplora_2020}.
% Thus, CoLoRa~\cite{colora} and NScale~\cite{tong_combating_2020} translate packet time offset into spectral peak ratio to concentrate energy on frequency spectrum, enabling collision resolving under low-SNR conditions.

% \emph{Fundamental limitations:} All existing collision resolving schemes~\cite{mLoRa,oct,xia2019ftrack,colora,tong_combating_2020,xu_fliplora_2020,eletreby2017empowering,hu2020sclora} are based on the adopted linear chirps of CSS modulation, which have two inherent limitations in decoding collided LoRa signals, including 1). SNR loss induced by phase-undetermined SIC~\cite{mLoRa,oct} or segmented symbols~\cite{colora,tong_combating_2020} and 2). stringent SIR requirements for collided signals~\cite{xia2019ftrack,tong_combating_2020}.
% As a result, those methods have a high SNR loss compared with the original LoRa decoding and only deal with collisions for power-comparable LoRa packets. 
% We further provide the theoretical analysis and experimental evaluations in $\S$\ref{sec-background}.

% \begin{figure}[t]
% \centering
% \subfigure[LoRa linear chirp]{
%     % \includegraphics[width=0.49\textwidth]{figures/LoRaModulation.pdf}
%     \includegraphics[width=0.49\textwidth]{figs/LoRaModulation.png}
%     \label{subfig-lora-chirp}
% }
% \subfigure[\ours non-linear chirps]{
% % 	\includegraphics[width=0.49\textwidth]{figures/CurvingLoRaModulation.pdf}
% 	\includegraphics[width=0.49\textwidth]{figs/CurvingLoRaModulation.png}
%     \label{subfig-currvelora-chirp}
% }
% \caption{An illustration of two concurrent transmissions modulated by (a) linear chirps and (b) non-linear chirps.}
% \label{fig-overview}
% \end{figure}

%\ours design
% \vspace{1mm}
% \noindent
% \textbf{Our Approach:} To resolve the collision fundamentally, we propose \ours, a physical layer technology, to boost LoRaWAN throughput with non-linear chirps (e.g., polynomial, logarithmic, exponential, trigonometric). Different with linear chirps, non-linear chirps demonstrate specific energy focusing effect in the standard demodulation scheme of LoRa ($\S$\ref{sec-design}), which can be explored to support extra orthogonality for collided signals. 
% Figure~\ref{fig-overview} illustrates the modulated linear chirps and collided non-linear chirps created by \ours. 
% In LoRa linear chirp modulation, as shown in Figure~\ref{subfig-lora-chirp}, a transmitter uses linear (e.g., blue solid lines) up-chirps starting from different frequencies to indicate different symbols. 
% In contrast, \ours is non-linear chirp based modulation, in which two transmitters deliver polynomial or exponential (e.g., red and green dashed curves) up-chirps to modulate symbols with the same SF with the linear ones. 
% Multiple transmissions modulated by the non-linear chirps can be demodulated simultaneously by using the standard demodulation scheme of LoRa with corresponding shaped down-chirps ($\S$\ref{subsec-design-1}). 

% \vspace{1mm}
% \noindent
% \textbf{Non-linearity meets Linearity:} In practice, \ours presents several specific characteristics, in which non-linear chirps are consistent or even outperform the linear chirps in noise and interference resilience. Thus, it captures the extra throughput gains by supporting more concurrent transmissions of packets in the same physical channel and SF setting.
% 1). In case of no collisions, non-linear chirp modulation demonstrates consistent throughput with the linear chirp modulation, under the same SF setting. Meanwhile, the SNR requirement of \ours symbol reception is as low as LoRa's regarding to environment noise  ($\S$~\ref{subsec-design-2}); 
% 2). When multiple packets are simultaneously transmitted and collided at the gateway, \ours is agnostic to the signal power difference of collided packets with a limited SNR loss, but weak signals are hard to be decoded or even received with linear chirps ($\S$~\ref{subsec-design-3}).
% 3). \ours verifies the non-linear chirps consumes comparable energy in our prototype, enabling its low-power deployment in the wild ($\S$~\ref{subsec-design-4}).


% To optimize LoRaWAN throughput by combining LoRa and \ours, we mainly address two challenging problems, delivering an end-to-end LoRa networking system based on the non-linear chirps ($\S$~\ref{sec-system}). 

% First, symbol time synchronization is a critical to align the received symbols for correct demodulation. In LoRa, symbol time misalignment incurs a linear frequency offset so that we can easily estimate the time offset to calibrate time synchronization. 
% In \ours, however, the resulted frequency offset is no longer linear. And the Central Frequency Offset (CFO) further leads extra interference which misleads symbol alignment. 
% We utilize a pair of up-chirp and down-chirp to develop a heuristic method which can accurately and effectively mitigate CFO and align received symbols ($\S$~\ref{subsec-symbol-alignment-demodulation}).

% Second, a logical channel has its own SNR requirement. Two logical channels are not orthogonal any more when the received signal strength of a transmission is much higher than the other's~\cite{Orthogonality}.
% We define a signal-to-interference ratio (SIR) metric to depict the interference between two logical channels ($\S$~\ref{subsubsec-logical-channel-interference}). Then, given a set of logical channels, to avoid negative influence brought by collisions across logical channels, we design an algorithm to select a subset of logical channels to maximize LoRaWAN throughput ($\S$~\ref{subsec-logical-channel-selection}).  

% We implement \ours with HackRF and USRP, then conduct extensive experiments and simulations to comprehensively evaluate its performance in various scenarios. The experimental results show that \ours can increase to 6.15$\times$ LoRaWAN throughput that only utilizing LoRa. The main contributions are summarized as follows:
% \begin{itemize}
%     \item We propose \ours which first use non-linear chirps to construct more logical channels so that significantly improves the ceiling of LoRaWAN throughput.
%     \item We develop a novel collision model between two logical channels, then select the optimal set of logical channels which can maximize network throughput.
%     \item We implement \ours on real hardwares and extensively evaluate its performance. The results show that LoRaWAN throughput can increase to 6.15$\times$.
% \end{itemize}



    

==> CurvingLoRa NSDI 22/3Preliminary.tex <==
\section{Motivation}
\label{sec-background}

In this section, we briefly introduce the LoRa physical layer and then analyze the pros and cons of linear chirps (\S\ref{subsec-background-2}). A discussion on the limitations of resolving linear-chirp LoRa collisions follows (\S\ref{subsec-background-3}).
%First, LoRa physical layer adopts the chirp spread spectrum and the "dechirp" as the standard symbol modulation and demodulation based on linear chirps. Second, linear chirps specifies certain properties, enabling significant noise resilience. While it suffers with collisions, in which two symbols from two different transmitters are overlapped. Third, existing approaches aim to resolve the collision for throughput gains but demonstrate inherent limitations from the linear chirps.

%LoRaPhy modulation and demodulation
\label{subsec-background-1}
\begin{figure}[t]
\centering
\subfigure[Baseline up-chirp]{ 
	\includegraphics[width=0.33\columnwidth]{figures/LoRaPrime1.pdf}
        \label{subfig-baseline-chirp}
}
\hspace{-0.06\columnwidth}
\subfigure[Shifted up-chirp]{
	\includegraphics[width=0.33\columnwidth]{figures/LoRaPrime22.pdf}
        \label{subfig-shifted-chirp}
}
\hspace{-0.06\columnwidth}
\subfigure[Symbol collision]{
	\includegraphics[width=0.33\columnwidth]{figures/LoRaPrime32.pdf}
        \label{subfig-symbol-collision}       
}
\vspace{-3mm}
\caption{LoRa PHY-layer design. 
{\normalfont 
(a): the multiplication of an up-chirp and a down-chirp leads to an energy peak on a specific FFT. (b): The position of this energy peak varies with the initial frequency offset of the incoming up-chirp. (c): Two collided symbols have separate energy peaks on FFT bins.}}
\label{fig-lora-preliminary}
\vspace{-3mm}
\end{figure}

\begin{figure*}[t] \label{fig:sic}
    \centering
    \subfigure[SER fluctuates with SNR in the absence of collisions.]{
    \includegraphics[width=0.495\columnwidth]{nsdi_figs_169/snr2ser_benchmark.pdf}
    \label{subfig-sic-1}
    }
    \hspace{-0.01\columnwidth}
     \subfigure[SER fluctuates with SNR in the presence of collisions.]{
    \includegraphics[width=0.495\columnwidth]{nsdi_figs_169/snr2ser_linear.pdf}
    \label{subfig-sic-2}
    }
   \hspace{-0.01\columnwidth}
     \subfigure[SER fluctuates with SIR in the presence of collisions.]{
    \includegraphics[width=0.495\columnwidth]{nsdi_figs_169/sir2ser_linear.pdf}
    \label{subfig-sic-3}
    }
    \hspace{-0.01\columnwidth}
    \subfigure[SER fluctuates with symbol offset in the presence of collisions.]{
    \includegraphics[width=0.495\columnwidth]{nsdi_figs_169/offset2ser_sic.pdf}
    \label{subfig-sic-4}	
    }
    \vspace{-4mm}
    \caption{Evaluation of the successive interference cancellation-based collision resolving method~\cite{mLoRa,eletreby2017empowering} in various settings.}
    \vspace{-4mm}
\end{figure*}


\paragraph{LoRa Physical Layer.}
LoRa modulates data with chirp spread spectrum (CSS)~\cite{berni1973utility, eletreby2017empowering}.
The transmitter encodes bits by varying the initial frequency offset of a standard up-chirp.\footnote{A chirp signal whose frequency grows linearly from $-{BW}/{2}$ to ${BW}/{2}$.}
%At the transmitter side, bit streams are encoded into symbols using chirps. 
For instance, bits `00' are encoded by an up-chirp with zero initial frequency offset, while bits `01' are encoded by shifting the initial frequency by $f_0$. The frequency component beyond ${BW}/{2}$ will be wrapped to $-{BW}/{2}$, ensuring full bandwidth occupancy.
%data bits can be encoded by shifting the initial frequency of a base up-chirp to $f_{0}$, rendering encoded chirp symbols as $y_e=h(t)e^{j 2 \pi f_0 t}$. 
%Shown in top Figure~\ref{subfig-shifted-chirp}, the start frequency of the modulated up-chirp is shifted up by $f_0$, and the frequencies higher than ${BW}/{2}$ are moved down $BW$, then start from $-{BW}/{2}$.
Upon the reception of a LoRa packet, the receiver multiplies each chirp symbol with a standard down-chirp (i.e., the conjugate of a standard up-chirp). The multiplication leads to an FFT peak in the frequency domain, which allows the receiver to demodulate LoRa symbols based on the position of FFT peaks.
Figure~\ref{fig-lora-preliminary}(a)-(b) shows an example.

% Spreading Factor (SF) and Bandwidth (BW) are used to balance the communication range and energy consumption of LoRa signal~\cite{colora,tong_combating_2020}. XXXX

%the standard demodulation scheme, the dechirp, first multiplies the shifted up-chirp symbol with the time synchronized baseline down-chirp, formulated as $h^*(t)h(t)e^{j 2 \pi f_0 t} = e^{j 2 \pi f_0 t}$.
%By applying Fast Fourier Transform (FFT), a single peak appears at FFT bin $b_0$ which corresponds to $f_0$ in frequency domain. 
%Meanwhile, the peak of demodulated baseline up-chirp appears at FFT bin 0. Thus, we can decoded the data bits by detecting the single energy peak on the spectrum, as shown in bottom Figure~\ref{subfig-baseline-chirp} and \ref{subfig-shifted-chirp}.

% \subsection{SF Logical Channel}
% \label{subsec-sf-logical-channel}

% In LoRaWAN, $SF$ is used to specific a series of discrete time and determine the time span $T$ of up-chirps and down-chirps. Specifically, an up-chirp consists of $2^{SF}$ chips (i.e., time slot unit) to represent $SF$ bits. Each chip lasts $\frac{1}{BW}$ second. Therefore, an up-chirp lasts for $\frac{2^{SF}}{BW}$ seconds.
% Given a fixed $BW$, LoRaWAN allows to adjust $T$ by setting $SF$ from 7 to 12. When $BW$ is 125kHz, it takes about 1ms and 32.8ms to transmit an up-chirp by setting $SF$ as 7 and 12.

% For two overlapped symbols using different $SF$s, the signal-interference-ratio (SIR) threshold of successful demodulation is reduced. Daniel et al.~\cite{Orthogonality} show that a symbol of SF7 can be successfully demodulated if the SIR is larger than -8dB when it overlaps with a symbol of SF8. The larger the SF a symbol has, the lower the required SIR is. The symbol with weaker received signal strength than other overlapped symbols still have the chance to be demodulated. In this way, LoRaWAN splits a physical channel to 6 logical channels which enable simultaneous reception and improve the capacity.

% For different $SF$ logical channel, the channel throughput is relate to $\frac{SF\times BW}{2^{SF}}$~\cite{gr-lora}. Although a large $SF$ allows symbol demodulation with low SIR, the channel throughput is sacrificed due to its longer time span of an up-chirp.

\subsection{The Pros and Cons of Linear Chirp}
\label{subsec-background-2}

%LoRa adopts linear up-chirps to modulate data. 
In essence, the aforementioned \emph{dechirp} converges the power of each LoRa symbol to a specific frequency point (\emph{i.e.}, an energy peak on an FFT bin), which allows the LoRa chirp to be decodable in extremely low SNR conditions (\emph{i.e.}, $-20$~dB).
As more LoRa nodes get involved, we are expected to see packet collisions at the receiver since LoRa nodes abide by the least-restrictive MAC protocol ALOHA.
To solve packet collisions, LoRaWAN~\cite{alliance2020lorawan} stipulates a set of spreading factors (SF) from seven to 12 and different bandwidths (\emph{i.e.}, 125/250/500~KHz). Therefore, LoRa packets with different SFs or bandwidths can transmit concurrently on the same frequency band.
The receiver uses down-chirps with different SFs to disambiguate these concurrent transmissions.
However, the capacity of this regulation is limited: it supports only 18 pairs of SF\&BW combinations~\cite{hessar2018netscatter}.

Collision happens when two concurrent transmissions use the same SF and bandwidth.
In this case, we are expected to see two energy peaks in two separate FFT bins, as shown in Figure~\ref{subfig-symbol-collision}.
In practice, due to the near-far issue, one transmission (e.g., packet $A$ in red) may experience a stronger attenuation than the other (e.g., packet $B$ in blue).
Hence the energy peak of $A$ tends to be weaker than that of $B$ in FFT bins.
Accordingly, the receiver will take $A$ as noise and demodulate $B$ only.
When $A$ and $B$ experience similar attenuations, the receiver can reliably demodulate neither of them because their individual energy peak may bury each other across different symbols.
In a nutshell, when two LoRa packets collide, only the strongest transmission can be correctly demodulated by LoRaWAN. 
Otherwise, no transmissions can be reliably demodulated. 




% \vspace{1mm}
% \noindent
% \textbf{Cons:} While in case of collisions, the focused energy peaks of linear chirps hinder the demodulation of multiple collided packets adversely. 
% Figure~\ref{subfig-symbol-collision} shows an aligned and weak target symbol (e.g., red solid line), which focuses all $N_0$ samples in the aligned FFT window with a low transmitter power. However, the corresponding energy peak can be distorted or even overwhelmed by the unaligned but strong interfered chirp symbol (e.g., blue dashed line).
% In other words, if the signal strength difference of the received symbols is large enough, only the symbol with stronger signals can be correctly demodulated. Otherwise, no symbol can be reliably demodulated at all. The symbol collision further leads LoRa packet loss so that degrades LoRaWAN capacity~\cite{mLoRa,xia2019ftrack}.

\subsection{Resolving Linear-Chirp LoRa Collisions}
\label{subsec-background-3}
 
% To combat collisions,
% a straightforward solution is Successive Interference Cancellation (SIC)~\cite{gollakota2009interference,mollanoori2013uplink,eletreby2017empowering,mLoRa}. 
% For instance, Choir~\cite{eletreby2017empowering} rebuilds each individual transmission by measuring the frequency offset and the channel.
% It then subtracts the strong transmission from the collisions and decodes the weaker one.
% Similarly, mLoRa~\cite{mLoRa} resolves collisions by starting with a collision-free chunk and then iteratively reconstructs and extracts each demodulated symbols. 
% However, both these two SIC-based approaches fail to work in low SNR (<0dB) conditions due to the following reasons.
% $\bullet$ First, due to Carrier Frequency Offset (CFO) and Sampling Frequency Offset (SFO), the phase of received chirp symbols is likely to distort by a certain degree.
% This phase distortion is critical to the success of signal recovery in SIC but is difficult to estimate in low SNR conditions~\cite{colora}.
% $\bullet$ Second, SIC suffers from hardware imperfections~\cite{tong_combating_2020}, which is common on low-end IoT devices. The symbol recovering error accumulates gradually and is likely to fail the SIC in the end. In addition, the impact of ambient RF noise on SIC, particularly the parameter estimation for signal reconstruction, gets exacerbated at low SNR conditions.

% To avoid the error-prone signal recovery in SIC, recent studies~\cite{colora,tong_combating_2020,hu2020sclora,xu_fliplora_2020} propose to transform time offset among collision symbols into amplitude gaps in frequency domain. This allows the receiver to leverage the amplitude variation of FFT peaks to demodulate concurrent transmissions. However, to make these methods work, the receiver has to misalign the observing window with the collision symbols by a certain degree, which sacrifices the processing gain brought by the chirp modulation.
% To mitigate this issue, NScale~\cite{tong_combating_2020} proposes to scale the energy peak of weak LoRa transmissions after FFT.
% However, it fails to work in low SIR conditions and thus does not scale down to the near-far deployment.

%The amplitude of FFT peak induced by each LoRa symbol is proportional to the signal samples of this LoRa chirp within the current observing window.
%For two concurrent transmissions, the overlapping ratio between the leading transmission and the observing window decreases as we gradually moving the observing window; thus we are expected to see a declining peak induced by this leading transmission.

% resolve collisions 
% by fully exploiting the special energy focusing peak of chirps on spectrum. For example, CoLoRa~\cite{colora} and NScale~\cite{tong_combating_2020} translates packet time offset into spectral peak ratio to concentrates energy from time-domain features. Since the height of the energy peak is proportional to the length of the segment ($\S$\ref{appendix-1}). However, the peak ratio between two consecutive FFT windows incurs two limitations. First, the reduced samples in a segmented window delivers a lower energy peak for the target packets, weakening the noise resilience of LoRa chirps. Second, the peak ratio requires two detective energy peaks with comparable powers of collided chirps (e.g., $SIR>-3dB$), which impairs its performance in the near-far situations with distributed strong and weak signals.


Section \ref{sec-related-work} overviews the current practice on resolving LoRa collisions and explains their pros and cons. In this section, we implement a state-of-the-art SIC-based system, mLoRa~\cite{mLoRa}, and examine its performance in various SNR and SIR conditions. Noting that we also compare with other SOTA systems in the evaluation part.
% Specifically, we superimpose two LoRa packets with controllable symbol offset.
% We then add white Gaussian noise and tune the amplitude of these two collided packets to emulate various SNR and SIR conditions, respectively.
Figure~\ref{subfig-sic-2} shows the symbol error rate (SER) in different SNR conditions.
We observe that to maintain a low symbol error rate (e.g., <0.1), the SNR of the received signal should be higher than $5dB$ -- $25dB$ higher than the minimum SNR requirement for demodulating a collision-free LoRa transmission.
Such a high SNR requirement sets a strong barrier to mLoRa's adoption since LoRa transmissions tend to be very weak after attenuation over a long distance.
We then plot the symbol error rate measured in different SIR settings in Figure~\ref{subfig-sic-3}.
The result shows that the symbol error rate grows dramatically with the decreasing SIR, indicating that mLoRa~\cite{mLoRa} cannot demodulate the targeting LoRa transmission in the presence of strong concurrent LoRa transmission.
We further evaluate the impact of the symbol offset on SER.
The result (Figure~\ref{subfig-sic-4}) shows that the SER grows with decreasing symbol offset, confirming our analysis. 
%This is due to the fact that the amplitude of the interfering FFT peak grows as this interfering LoRa chirp gradually aligns with the observing window.

\vspace{1mm}
\noindent
\textbf{Remarks.} The above analysis reveals that the linear chirp in LoRaWAN does not scale to concurrent LoRa transmissions.
Although the state-of-the-arts have proposed various approaches to resolve LoRa collisions, most of them function only in good SNR or SIR conditions and thus sacrifice the precious processing gain brought by the chirp modulation.

%Illustrated in Figure~\ref{subfig-sic-2}, SIC based approach first weakens the noise resilience of linear chirps, rendering a higher SER in the same SNR with Figure~\ref{subfig-sic-1}. And it is consistent with the SNR requirement proposed by mLoRa~\cite{mLoRa}. Further, SIC suffers when the target signal gets weaker and weaker, with a lower SIR in Figure~\ref{subfig-sic-3}. Third, we study the impact of the symbol offset on the collision resolving. Figure~\ref{subfig-sic-4} shows the SER increases with a smaller offset between these two collided packets. And it can be attributed to the remaining peaks of the strong signals after SIC, distorting the weak signals for demodulation.

==> CurvingLoRa NSDI 22/4Design.tex <==
\section{Analysis: Non-linear vs. Linear Chirps}
\label{sec-design}

We now show that by replacing the linear chirp with its non-linear counterpart, we can boost the capacity of concurrent transmissions (\S\ref{subsec-design-1}) while allowing the receiver to demodulate collision signals in severe SIR conditions (\S\ref{subsec-design-2}).
In addition, we show by both theoretical analysis and empirical validation that such a non-linear chirp design sacrifices neither noise resilience (\S\ref{subsec-design-3}) nor power efficiency (\S\ref{subsec-design-4}).

% In this section, we propose the basis of \ours, the specially designed non-linear chirps. Instead of using linear chirps for modulation and demodulation of LoRa, we first present the specific properties of non-linear chirps ($\S$\ref{subsec-design-1}), enabling a larger number of concurrency, even under the near-far effect. Besides, $\S$\ref{subsec-design-1} demonstrates non-linear chirps retain the advantages of linear chirp based CSS on its noise resilience. Finally, we compare the energy consumption between linear and non-linear chirps based on our prototype.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=3.2in]{./figures/fig_demodulation.pdf}
%     \vspace{-4mm}
%     \caption{(a): The receiver takes advantage of the power scattering effect to demodulate two collision symbols. (b): an illustration of demodulating five collision symbols.}
%     \label{fig:demodulation}
%     \vspace{-4mm}
% \end{figure}

\begin{figure}[t]
    \centering
    \subfigure[]{ 
	    \includegraphics[width=3.2in]{figures/fig_demodulation_1.pdf}
        \label{subfig-nonlinear-vs-linear-sir-1}
    }\\\vspace{-4.2mm}
    \subfigure[]{
    	\includegraphics[width=3.2in]{figures/fig_demodulation_2.pdf}
    	\label{subfig-nonlinear-vs-linear-sir-2}
    }
    \vspace{-4mm}
    \caption{(a): The receiver takes advantage of the power scattering effect to demodulate two collision symbols. (b): an illustration of demodulating five collision symbols.}
    \label{fig:demodulation}
    \vspace{-4mm}
\end{figure}

%illustrate non-linear chirps have low SIR theoretically and empirically
% \begin{figure}[t]
% \centering
% \subfigure[Aligned Spectrum]{
% \includegraphics[width=0.23\textwidth]{figs/aligned.pdf}
% \label{subfig-aligned}
% }
%  \hspace{-0.04\columnwidth}
% \subfigure[Misaligned Spectrum]{
% \includegraphics[width=0.23\textwidth]{figs/misaligned.pdf}
% \label{subfig-misaligned}
% }
%  \hspace{-0.04\columnwidth}
% \subfigure[Two Chirps' Collision]{
% \includegraphics[width=0.23\textwidth]{figs/two-collision.pdf}
% \label{subfig-two-collision}
% }
%  \hspace{-0.04\columnwidth}
% \subfigure[Five Chirps' Collision]{
% \includegraphics[width=0.23\textwidth]{figs/multi-collision.pdf}
% \label{subfig-multi-collision}
% }
% \vspace{-3mm}
% \caption{An illustration of energy converging and scattering effect. 
% {\normalfont
% (a) The energy of a non-linear chirp symbol converges to a single frequency point when it is well aligned with the down-chirp (the observing window). (b) The energy of a non-linear chirp symbol scatters to multiple frequency points when it is not well aligned with the down-chirp. (c) The receiver takes  advantage of power scattering effect to demodulate two collision symbols. (d) Demodulating five collision symbols.}}
% \label{fig-non-linear-collision}
% \vspace{-3mm}
%\subfigure{
%    \includegraphics[width=0.8\columnwidth]{figs/collision_linear.png}
%    \label{subfig-nonlinear-vs-linear-1}
%}

% \hspace{-0.06\columnwidth}
%\\
%\subfigure{
%	\includegraphics[width=0.8\columnwidth]{figs/collision_curving.png}
%    \label{subfig-nonlinear-vs-linear-2}
%}
%\caption{Linear (top) v.s. Non-linear Chirps (bottom) on focusing and spreading energy for unaligned packets.}
%\label{fig-nonlinear-vs-linear}
%\end{figure}

% \begin{figure*}[t]
%     \centering
%     \subfigure[Collisions of linear chirps]{
%     \includegraphics[width=0.49\columnwidth]{figs/sir2peak_1_0.6.png}
%     \label{subfig-nonlinear-vs-linear-pre-1}
%     }
%     \hspace{-0.06\columnwidth}
%       \subfigure[SNR=+$\infty$, SIR=-1dB]{
%     \includegraphics[width=0.49\columnwidth]{figs/sir2peak_1_peak.png}
%     \label{subfig-nonlinear-vs-linear-pre-2}
%     }
%     \hspace{-0.06\columnwidth}
%       \subfigure[$t_{gap}$=30\%, SIR=-1dB]{
%     \includegraphics[width=0.49\columnwidth]{figs/sir2peak_1_snr.png}
%     \label{subfig-nonlinear-vs-linear-pre-3}
%     }
%     \hspace{-0.06\columnwidth}
%     \subfigure[$t_{gap}$=30\%, SNR=+$\infty$]{
%     \includegraphics[width=0.49\columnwidth]{figs/sir2peak_1_sir.png}
%     \label{subfig-nonlinear-vs-linear-pre-4}	
%     }
%     \subfigure[Collisions of non-linear chirps]{
%     \includegraphics[width=0.49\columnwidth]{figs/sir2peak_2_0.6.png}
%     \label{subfig-nonlinear-vs-linear-pre-5}
%     }
%     \hspace{-0.06\columnwidth}
%       \subfigure[SNR=+$\infty$, SIR=-1dB]{
%     \includegraphics[width=0.49\columnwidth]{figs/sir2peak_2_peak.png}
%     \label{subfig-nonlinear-vs-linear-pre-6}
%     }
%     \hspace{-0.06\columnwidth}
%       \subfigure[$t_{gap}$=30\%, SIR=-1dB]{
%     \includegraphics[width=0.49\columnwidth]{figs/sir2peak_2_snr.png}
%     \label{subfig-nonlinear-vs-linear-pre-7}
%     }
%     \hspace{-0.06\columnwidth}
%     \subfigure[$t_{gap}$=30\%, SNR=+$\infty$]{
%     \includegraphics[width=0.49\columnwidth]{figs/sir2peak_2_sir.png}
%     \label{subfig-nonlinear-vs-linear-pre-8}	
%     }
%     \label{fig-nonlinear-vs-linear-pre}
%     \caption{Linear vs non-linear on noise resilience: resolving collisions with various SNRs and symbol offsets.}
% \end{figure*}
\begin{figure*}[t]
    \centering
    \subfigure[L. chirp collisions in time domain]{
    \includegraphics[width=0.515\columnwidth]{nsdi_figs_169/sir2peak_1_0.6_abs_note.png}
    \label{subfig-nonlinear-vs-linear-pre-1}
    }
    %\hspace{-0.06\columnwidth}
      \subfigure[L. chirp collisions in freq.]{
    \includegraphics[width=0.475\columnwidth]{nsdi_figs_169/sir2peak_1_sir_abs.pdf}
    \label{subfig-nonlinear-vs-linear-pre-2}
    }
    %\hspace{-0.06\columnwidth}
      \subfigure[NL. chirp collisions in time domain]{
    \includegraphics[width=0.515\columnwidth]{nsdi_figs_169/sir2peak_2_0.6_abs.png}
    \label{subfig-nonlinear-vs-linear-pre-3}
    }
    %\hspace{-0.06\columnwidth}
    \subfigure[NL. chirp collisions in freq.]{
    \includegraphics[width=0.475\columnwidth]{nsdi_figs_169/sir2peak_2_sir_abs.pdf}
    \label{subfig-nonlinear-vs-linear-pre-4}	
    }
    % \vspace{-4mm}
    \caption{Comparison of linear and non-linear chirps on resolving the near-far issue. 
    {\normalfont
    (a): Three linear chirps with different SNR collide at the receiver. (b): Due to the near-far issue, the energy peak (in black) of the weak reception is overwhelmed by the energy peaks (in red) of strong collision symbols. (c): Three non-linear chirps in the same collision situations. (d): The spectral power of strong receptions is spread over multiple frequency points, making the corresponding FFT peaks (in red) significantly lower than the converged power (in black) of the weak reception.}}
    \label{fig-nonlinear-vs-linear-pre}
    \vspace{-4mm}
\end{figure*}

\subsection{Non-linear Chirps Meet Collisions}
\label{subsec-design-1}

We define a non-linear up-chirp as a signal whose frequency grows non-linearly from $-BW/2$ to $BW/2$. The non-linear function can be either polynomial, logarithmic, exponential, or trigonometric.
The receiver operates dechirp to demodulate non-linear chirp symbols.

%\vspace{1mm}
% \noindent
% \textbf{Energy scattering and converging effect.} Similar to the linear up-chirp, when a non-linear up-chirp is well aligned with its down-chirp counterpart in the current observing window, the multiplication of these two signals {\it converges} the power of the up-chirp signal to a specific frequency point, resulting in an FFT peak (shown in Figure~\ref{subfig-aligned}). 
% In contrast, when these two chirps are not well aligned on the observing window  (i.e., with few samples offset), the dechirp operation will {\it scatter} the power of this up-chirp into multiple FFT bins (shown in Figure~\ref{subfig-misaligned}).
% Such energy scattering effect will show up as long as the non-linear up-chirp is not well aligned with the down-chirp (The theoretical analysis is in Appendix \ref{appendix-2}). 


%An intuitive explanation is that the misalignment between a non-linear chirp and the base down-chirp makes the multiple frequency components incurred by the non-linearity cannot be fully mitigated by ``dechirping'' them together.
%The detailed theoretical analysis is omitted to conserve space.
%as we proved in Appendix~\ref{appendix-2}. 

\vspace{1mm}
\noindent
Considering two collision symbols $A$ and $B$, as shown in Figure~\ref{fig:demodulation}(a).
The receiver takes a sliding window approach to demodulate incoming signals.
As aforementioned, when symbol $A$ aligns with the down-chirp in the current observing window, we are expected to see a strong energy peak (termed as peak $A$) on the associated FFT bin.
At the same time, the energy of symbol $B$ will be spread over multiple, clustered FFT bins due to its misalignment with the down-chirp.
Compared to peak $A$, the amplitude of these clustered energy peaks is significantly weaker.
The receiver inherently takes these clustered FFT peaks as noise and demodulates symbol $A$.
As the observing window slides, symbol $B$ will align with the down-chirp at a time.
Consequently, the dechirp converges the power of symbol $B$ to a specific frequency point while spreading the power of symbol $A$ into multiple frequency bins instead.
The receiver then takes symbol $A$ as noise and demodulates $B$.
When it comes with two collision packets with each consisting of tens of symbols, following the same principle, the receiver slides the observing window step by step and demodulates their individual symbols alternatively.

\vspace{1mm}
\noindent
\textbf{Remarks.} In essence, when the collision symbols are not strictly aligned, there will be only one symbol that aligns with the down-chirp in each observing window.
This indicates that each time only one symbol gets its energy accumulated while the energy of all the other colliding signals is being scattered over multiple FFT bins, as shown in Figure~\ref{fig:demodulation}(b).
Hence the receiver can easily pick up each individual symbol on separated observing windows and decode them chronologically.


%Figure~\ref{} shows five symbols modulated by different types of chirps collide at the receiver. 
%When these symbols are all modulated by linear chirps,
%we observe five isolated peaks after FFT operation and the receiver can only demodulate the strongest one. 
%In contrast, when these five symbols are modulated by non-linear chirps, each time only one symbol will be de-spread on a specific frequency point while all the others are scattered into multiple frequency bins. The receiver can thus demodulate each individual symbols chronologically.

% \vspace{1mm}
% \noindent
% \textbf{Theoretical Analysis:} In comparison with linear chirps, the frequency of a based non-linear chirp denotes grows ``non-linearly'' over time from $-BW/2$ to $BW/2$, which can be polynomial, logarithmic, exponential, or trigonometric. On one hand, a non-linear chirp keeps the spectral energy focusing when aligned with the FFT window, rendering the same noise resilience by suppressing the accumulated noise energy. On the other hand, an unaligned non-linear chirp spreads out the energy along the spectrum instead of focusing the segmented symbol at a single tone via linear chirps.

% We illustrate the difference between linear and non-linear chirps in Figure~\ref{fig-nonlinear-vs-linear}, in which the energy spreading effect of non-linear chirps help resolve the collisions. 
% $\S$~\ref{subsec-background-2} first demonstrates the height of the energy peak of a linear chirp is the product of the amplitude $h$ of the received symbol and the length of the segment $N_0$ located in the FFT window. Thus we can observe three comparable energy peaks on the spectrum of collided linear chirps in Figure~\ref{subfig-nonlinear-vs-linear-1}. For the correct demodulation of LoRaWAN, the peak $p_1$ of the target symbol has to be larger than the interfered ones, such as $p_a$ and $p_b$, which is determined by the offset and the power difference between three collided symbols.

% When non-linear chirps meet the collision, however, the spectral energy can be focused or spread, depending on the FFT window is aligned with the chirp symbol or not. Shown in Figure~\ref{subfig-nonlinear-vs-linear-2}, the collision occurs among non-linear chirps with the same collision offset and power distribution. For the target chirp symbol 1, an aligned FFT window renders a corresponding spectral energy peak while spreading the spectral energy of both two interfered chirp symbols on the spectrum, rendering a series of much lower peaks along the spectrum. To ensure the correct demodulation of the target chirp, the focused energy peak $p_1$ only needs to be larger than any of the low peaks $p_{ai}$ and $p_{bj}$. Due to the energy spreading of the unaligned non-linear chirp, the target symbol can be decoded easily, even its power is much lower than the unaligned interfered symbols.

% \vspace{1mm}
% \noindent
% \textbf{Preliminary Evaluation:} To verify what happened when non-linear chirps meet collision, we simulate the corresponding encoded linear and non-linear chirps with Figure~\ref{fig-nonlinear-vs-linear} in our general modulation framework ($\S$~\ref{subsec-system-1}), in which the frequency of the former grows linearly over time (e.g., $y(t)=kt$) while the latter increases quadratically (e.g., $y(t)=kt^2$). 
% Figure~\ref{subfig-nonlinear-vs-linear-pre-1} and \ref{subfig-nonlinear-vs-linear-pre-4} first illustrate the two kinds of collisions on the spectrogram, corresponding the aligned FFT window in Figure~\ref{fig-nonlinear-vs-linear}. 
% After the standard demodulation, three consecutive spectral peaks can be observed clearly in Figure~\ref{subfig-nonlinear-vs-linear-pre-2} with the give symbol offsets (e.g., 30\%, 50\%, and 60\%) while Figure~\ref{subfig-nonlinear-vs-linear-pre-6} only reports a single energy peak corresponding to the aligned target chirp symbol, with a much lower energy plateau of the interfered non-linear chirps. Besides, it is resilient to the symbol offset between the collided symbols, which can affect the height of peaks for interfered linear chirps.

\subsection{Accounting for the Near-far Effect}
\label{subsec-design-2}

The above section explains the basic idea of non-linear chirp and its unique energy scattering effect, we next demonstrate that this energy scattering effect can be leveraged to address the {\it near-far issue} where weak receptions are buried by strong receptions from nearby transmitters.

Consider a large number of colliding transmitters where some are physically closer to the receiver compared to the others.
When linear chirps are adopted, the power of strong receptions {\it converges} to a specific frequency point where the associated energy peak is easily distinguishable after dechirp.
The weak receptions from remote transmitters, however, have significantly weaker energy peaks.
The receiver thus takes those weak receptions as noise.
Figure~\ref{subfig-nonlinear-vs-linear-pre-1} shows a snapshot where two linear chirp packets with a distinguishable SIR (-10dB) collide at the receiver.
Suppose the current observing window aligns with the symbol $A$ in yellow of the weak packet.
Due to the near-far issue, symbol $B$ and $C$ in red produce stronger energy peaks on associated FFT bins even they both are not aligned with the current observing window (shown in Figure~\ref{subfig-nonlinear-vs-linear-pre-2}).
Hence the receiver cannot demodulate symbol $A$ successfully.
In contrast, when non-linear chirps are adopted (shown in Figure~\ref{subfig-nonlinear-vs-linear-pre-3}), the power of strong reception symbols $B$ and $C$ are both {\it scattered} into multiple FFT bins after dechirp.
Due to such an energy scattering effect, the energy peaks induced by these strong symbols become lower than the accumulated energy peak induced by the weak symbol $A$. This allows the receiver to demodulate symbol $A$ in the presence of strong collision symbols $B$ and $C$ (shown in Figure~\ref{subfig-nonlinear-vs-linear-pre-4}).

\begin{figure}[t]
\centering
\subfigure[SER of linear and non-linear chirps in different SIR conditions.]{ 
	    \includegraphics[width=0.22\textwidth]{nsdi_figs_169/sir2map_fs125k_SF10_sir2ser_sine_v4.pdf}
        \label{subfig-nonlinear-vs-linear-sir-1}
}
\hspace{-0.02\columnwidth}
\subfigure[The SIR threshold for linear and non-linear chirps to achieve 1\% SER.]{
	\includegraphics[width=0.22\textwidth]{nsdi_figs_169/sir2map_fs125k_SF_bar_sine_part_optimal_v2.pdf}
	\label{subfig-nonlinear-vs-linear-sir-2}
}
\vspace{-3mm}
\caption{Comparing the SER of linear and non-linear chirps in various near-far conditions.}
\label{fig-nonlinear-vs-linear-sir}
\vspace{-4mm}
\end{figure}


\begin{figure*}[t]
    \centering
    \subfigure[Two collided linear chirps]{
    \includegraphics[width=0.53\columnwidth]{nsdi_figs_169/sir2peak_1_0.6_tgap_note.png}
    \label{subfig-nonlinear-vs-linear-tgap-1}
    }
    \hspace{-0.06\columnwidth}
      \subfigure[SIR=-1dB]{
    \includegraphics[width=0.49\columnwidth]{nsdi_figs_169/sir2peak_1_-1_peak_tgap.pdf}
    \label{subfig-nonlinear-vs-linear-tgap-2}
    }
    \hspace{-0.06\columnwidth}
      \subfigure[SIR=-5dB]{
    \includegraphics[width=0.49\columnwidth]{nsdi_figs_169/sir2peak_1_-5_peak_tgap.pdf}
    \label{subfig-nonlinear-vs-linear-tgap-3}
    }
    \hspace{-0.06\columnwidth}
    \subfigure[SIR=-10dB]{
    \includegraphics[width=0.49\columnwidth]{nsdi_figs_169/sir2peak_1_-10_peak_tgap.pdf}
    \label{subfig-nonlinear-vs-linear-tgap-4}	
    }\vspace{-3mm}
    \subfigure[Two collided non-linear chirps]{
    \includegraphics[width=0.53\columnwidth]{nsdi_figs_169/sir2peak_2_0.6_tgap_note.png}
    \label{subfig-nonlinear-vs-linear-tgap-5}
    }
    \hspace{-0.06\columnwidth}
      \subfigure[SIR=-1dB]{
    \includegraphics[width=0.49\columnwidth]{nsdi_figs_169/sir2peak_2_-1_peak_tgap.pdf}
    \label{subfig-nonlinear-vs-linear-tgap-6}
    }
    \hspace{-0.06\columnwidth}
      \subfigure[SIR=-5dB]{
    \includegraphics[width=0.49\columnwidth]{nsdi_figs_169/sir2peak_2_-5_peak_tgap.pdf}
    \label{subfig-nonlinear-vs-linear-tgap-7}
    }
    \hspace{-0.06\columnwidth}
    \subfigure[SIR=-10dB]{
    \includegraphics[width=0.49\columnwidth]{nsdi_figs_169/sir2peak_2_-10_peak_tgap.pdf}
    \label{subfig-nonlinear-vs-linear-tgap-8}
    }
    % \vspace{-4mm}
    \caption{Examining the resilience to symbol time offset in different symbol-to-interference ratio settings.}
    \label{fig-nonlinear-vs-linear-tgap}
    \vspace{-4mm}
\end{figure*}

\vspace{1mm}
\noindent
\textbf{Validation.} To demonstrate the effectiveness of non-linear chirps on resolving the near-far issues, we compare the symbol error rate of non-linear and linear chirps in different signal-to-interference ratio (SIR) settings.
The spreading factor, bandwidth, and sampling rate are set to 10, 125KHz, and 1MHz, respectively.

Figure~\ref{subfig-nonlinear-vs-linear-sir-1} shows the results. 
In accordance with our analysis, we observe that the linear chirp fails to demodulate the targeting symbol in the presence of strong concurrent transmissions (i.e., SER=100\% when SIR<$-5dB$). 
The SER then drops to around 10\% when the power of the targeting symbol is comparable to that of colliding symbols (i.e., SIR=$0dB$).
In contrast, the receiver can successfully demodulate the weak non-linear symbols as long as the SIR is higher than $-25dB$.
We also found that the non-linear chirp can still achieve $10\%$+ SER in an extreme case where the colliding signal is $20dB$ stronger than the targeting signal (i.e., SIR=$-20dB$).
The SER drops dramatically to 1\% as the SIR decreases from $-20dB$ to $-10dB$.
We further evaluate the SER in different spreading factor settings.
Figure~\ref{subfig-nonlinear-vs-linear-sir-2} shows the minimum SIR required by each type of chirps in order to achieve less than 1\% symbol error rate.
We observe that the linear chirp requires a minimal SIR of around $0dB$ in all six spreading factor settings.
In contrast, the non-linear chirps require a minimal SIR less than $0dB$, and the SIR requirement drops dramatically with increasing spreading factor. 
These results clearly demonstrate that the non-linear chirp by its own design is more scalable to near-far issues than its linear chirp counterpart.


\vspace{1mm}
\noindent
\textbf{The impact of symbol time offset.} We define $t_{gap}$ as the symbol time offset between two colliding symbols $A$ and $B$ (shown in Figure~\ref{subfig-nonlinear-vs-linear-tgap-1}).
Suppose the current observing window aligns with symbol $A$, then after dechirping, the power of the interfering symbol $B$ will be scattered into multiple FFT bins.
The amplitude of these scattered FFT peaks  is proportional to 1-$t_{gap}$ because only those signal samples that are within the overlapping window will contribute to the energy peaks.
Hence a smaller $t_{gap}$ will lead to stronger interfering peaks.
We vary $t_{gap}$ and plot the energy peaks in Figure~\ref{fig-nonlinear-vs-linear-tgap}.

Figure~\ref{subfig-nonlinear-vs-linear-tgap-2} shows the energy peaks of linear chirps. When SIR=$-1dB$, the targeting peak is still distinguishable from the interfering  peak across all four $t_{gap}$ settings.
When SIR drops to $-5dB$ (shown in Figure~\ref{subfig-nonlinear-vs-linear-tgap-3}), the interfering peak grows dramatically with decreasing $t_{gap}$. It finally surpasses the targeting peak when $t_{gap}$ drops to 20\%.
When SIR grows to -10$dB$ (shown in Figure~\ref{subfig-nonlinear-vs-linear-tgap-4}), the interfering peak easily exceeds the targeting peak in 3/4 $t_{gap}$ settings.
In contrast, when a non-linear chirp is adopted, we merely observe tiny energy peaks induced by the interfering symbol $B$. The targeting peak is easily distinguishable even in the case that the colliding symbol B is almost aligned with the targeting symbol A (i.e., $t_{gap}$=20\%) across all three SIR settings, as shown in  Figure~\ref{subfig-nonlinear-vs-linear-tgap-6}-(h).
These results manifest that the non-linear chirp is robust to symbol time offset. In \S\ref{subsec-system-1} we further demonstrate that by adopting different forms of non-linear chirps, the receiver can even demodulate two well-aligned collision symbols (i.e., $t_{gap}$=0) --- a case that none of existing LoRa collision demodulation approaches can deal with.

%even in the extreme case where two collision symbols overlapped with each other by \textcolor{red}{XX}$\%$, the amplitude of those scattered energy peaks are still significantly lower than the energy peak induced by the targeting signal (i.e., the one well aligned with the current observing window). The receiver thus can reliably demodulate this targeting signal.
%In contrast, the state-of-the-art \textcolor{red}{describing the performance}.


% \vspace{1mm}
% \noindent
% \textbf{Validation:} To demonstrate the effectiveness of non-linear chirps on resolving the near-far issues, we evaluate the symbol error rate of six types of non-linear chirps in different signal-to-interference ratio (SIR) settings.
% haThese six types of non-linear chirps cover a range of shapes and convexity, and can be easily generated by the following polynomial functions (\S\ref{subsec-system-1}): $quadratic1$---$f(t) = t^2$, $quadratic2$---$f(t) = -t^2+2t$, $quartic1$---$f(t) = t^4$, $quartic2$---$f(t) = -t^4+4t^3-6t^2+4t$, $Sine1$---$f(t) = sin(t),t\in[-\pi/2,\pi/2)$, and $Sine2$---$f(t) = sin(t),t\in[-3\pi/8,3\pi/8)$.
% The spreading factor is set to 12 across all experiments.

% Figure~\ref{fig-nonlinear-vs-linear-sir} shows the results. 
% In accordance with our analysis, we observe that the linear chirp fails to demodulate the targeting symbol in the presence of strong concurrent transmissions (i.e., SER=100\% when SIR<$0dB$). 
% The SER then drops to around 1\% when the power of targeting symbol is compatible to that of collision symbols (i.e., SIR=$0dB$).
% In contrast, all six types of non-linear chirps can successfully demodulate the weak targeting signal in the presence of strong collisions.
% Taking a step further, we found that the non-linear chirp produced by $Quandratic-1$ achieves an SIR of 1\% when the collision signal is $25dB$ stronger than the targeting signal (i.e., SIR=$-25dB$).
% The SER drops dramatically to 0.1\% and 0.01\% as the SIR decreases from $-25dB$ to $-15dB$ and further to $-5dB$.
% The other five types of non-linear chirps all show the similar SER trend.
% We further evaluate the SER of these six groups of non-linear chirps (plus the linear chirp for comparison) in different spreading factor settings.
% Figure~\ref{subfig-nonlinear-vs-linear-sir-2} shows the minimum SIR required by each individual types of chirps in order to achieve less than 1\% symbol error rate.
% We observe that the linear chirp requires a minimal SIR of around $0dB$ SIR in all six spreading factor settings.
% In contrast, all six groups of non-linear chirps require a minimal SIR less than $0dB$, and this value further drops significantly with an increasing spreading factor. 
% These results clearly demonstrate that the non-linear chirps by their own design are more scalable to near-far issues than their linear counterpart.

% We have two takeaways from these experiment results. $i):$ The non-linear chirps provide us extra processing gain to deal with the near-far issues.
% $ii):$ The capability of handling near-far issues varies with the types of non-linear chirps. The transmitter thus can 


% -------------------

% Given teams of collided chirp symbols with random encoded data and offsets, we first adjust the SIRs elaborately to emulate various degrees of the near-far effect. And the SER trends of SIR are compared for the linear chirp and 6 other non-linear chirps in Figure~\ref{subfig-nonlinear-vs-linear-sir-1}. And weak signals (e.g., SIR<0dB) can be easily overwhelmed in collisions of linear chirps and have to be re-transmitted. 
% However, non-linear chirps harvest significant SIR gains by decreasing the SER for $SIR\in[-20dB,0dB)$, alleviating the near-far effect effectively.
% We further compute and compare the SIR threshold for different configurations of SF in Figure~\ref{subfig-nonlinear-vs-linear-sir-2}, under which the SER is no less than 1\% any more. It shows that the target chirps can be decoded reliably, even weaker than the collided chirps at the SIR of $-15dB$ for the Quadratic1 (e.g., $f(t)=t^2$) under $SF=12$. 
% Various SIR gains can implied and attributed to the similarity between the specific non-linear and linear chirp, which are studied in \S\ref{subsec-system-4}.

% -------------------------------

% the near-far effect hinders the weak signal decoding since those remote transmitters may have significantly weaker spectral energy peaks that are easily buried by those strong energy peaks from transmitters close to the receiver.
% Figure~\ref{subfig-nonlinear-vs-linear-pre-4} illustrates the overwhelmed spectral peak of the target chirp symbol in collisions, in which, the unaligned interfered chirp symbol is strong enough to distort (e.g., SIR=-3dB) or even suppress (e.g., SIR=-5dB) the target peak.
% While non-linear chirps can eliminate these interfered signals inherently by spreading out the energy on the spectrum. 
% Shown in Figure~\ref{subfig-nonlinear-vs-linear-pre-8}, the energy plateau of interfered chirps can only be elevated slightly as the SIR decreases between the target and interfered chirp symbols. Thus non-linear chirps are agnostic to the near-far effect, with readily discernible spectral energy peaks for weak target signals.

% \vspace{1mm}
% \noindent
% \textbf{Preliminary Evaluation:} Figure~\ref{fig-nonlinear-vs-linear-sir} demonstrates the quantitative SIR gains captured by different kinds of non-linear chirps. Given teams of collided chirp symbols with random encoded data and offsets, we first adjust the SIRs elaborately to emulate various degrees of the near-far effect. And the SER trends of SIR are compared for the linear chirp and 6 other non-linear chirps in Figure~\ref{subfig-nonlinear-vs-linear-sir-1}. And weak signals (e.g., SIR<0dB) can be easily overwhelmed in collisions of linear chirps and have to be re-transmitted. 
% However, non-linear chirps harvest significant SIR gains by decreasing the SER for $SIR\in[-20dB,0dB)$, alleviating the near-far effect effectively.
% We further compute and compare the SIR threshold for different configurations of SF in Figure~\ref{subfig-nonlinear-vs-linear-sir-2}, under which the SER is no less than 1\% any more. It shows that the target chirps can be decoded reliably, even weaker than the collided chirps at the SIR of $-15dB$ for the Quadratic1 (e.g., $f(t)=t^2$) under $SF=12$. 
% Various SIR gains can implied and attributed to the similarity between the specific non-linear and linear chirp, which are studied in \S\ref{subsec-system-4}.

%illustrate non-linear can performance as the same as linear in terms of SNR limits
\subsection{Noise Tolerance}
\label{subsec-design-3}

\begin{figure}[t]
\centering
\subfigure[SER fluctuates with SNR in various spreading factor settings.]{ 
	    \includegraphics[width=0.22\textwidth]{nsdi_figs_169/snr2ser_fs125k_type7_v4.pdf}
        \label{subfig-nonlinear-vs-linear-noise-1}
}
% \hspace{-0.1\columnwidth}
\subfigure[The CDF of SER in various spreading factor settings.]{
	\includegraphics[width=0.22\textwidth]{nsdi_figs_169/code2ser_fs125k_SF.pdf}
        \label{subfig-nonlinear-vs-linear-noise-2}
}
\vspace{-3mm}
\caption{Comparing the SER of various types of non-linear chirps in different SNR conditions.}
\label{fig-nonlinear-vs-linear-noise}
\vspace{-4mm}
\end{figure}

%\vspace{1mm}
%\noindent
%\textbf{Theoretical Analysis:} 

We next demonstrate that the non-linear chirp achieves the same noise tolerance as the linear chirp counterpart does.

%Non-linear chirps spread its spectral energy when it is misaligned with the observing window. 
%It however converges the energy of well aligned chirp symbol to a specific frequency point as linear chirp does after dechirp.
%This allows the receiver to demodulate the non-linear chirp in SNR conditions as low as linear chirp does, as we demonstrated below.

% retains the energy focusing when aligning with the FFT windows, which guarantees its comparable noise resilience with linear chirps. By suppressing the accumulated noise energy on the spectrum, non-linear chirps also achieve robust communication, even under low SNRs (e.g., -20dB). 
% We illustrate the spectral energy peak distribution of collided chirps in Figure~\ref{subfig-nonlinear-vs-linear-pre-3}, in which the spectral energy peak (e.g., frequency bin = 64) can be detected readily for the target linear chirps. 
% However, under SNR=-20dB, the accumulated noise energy can be enhanced by the focused energy peak of interfered symbols for linear chirps (e.g., frequency bin = 72), making it overwhelm the target peak adversely.
% Due to the energy spreading of non-linear chirps, the impact of interfered symbols can be amortized and minimized for the correct dechirp processing, shown in Figure~\ref{subfig-nonlinear-vs-linear-pre-7}.

\vspace{1mm}
\noindent
\textbf{Validation.} We evaluate the noise tolerance of six non-linear chirps that cover a range of shapes and convexity (\S\ref{subsec-system-1}): 
\vspace{-0.15in}
\begin{table}[h]
\small
\centering
\begin{adjustbox}{width=1\columnwidth}
\begin{tabular}{ll}
\hline 
 (1): $quadratic1$---$f(t) = t^2$ & (2): $quadratic2$---$f(t) = -t^2+2t$ \\
%\hline 
 (3): $quartic1$---$f(t) = t^4$ & (4): $quartic2$---$f(t) = -t^4+4t^3-6t^2+4t$ \\
 (5): $Sine1$---$f(t) = sin(t),t\in[-\pi/2,\pi/2)$ & (6): $Sine2$---$f(t) = sin(t),t\in[-3\pi/8,3\pi/8)$ \\
\hline 
\end{tabular}
\end{adjustbox}
\vspace{-0.15in}
\end{table}

Figure~\ref{subfig-nonlinear-vs-linear-noise-1} shows the SER achieved by these chirps in three spreading factor settings.
We observe that all these six types of non-linear chirps achieve consistent symbol error rates with their linear chirp counterpart across all three different spreading factor settings.
In particular, when $SF=11$, the receiver achieves 1\% SER on both non-linear and linear chirps in an extremely low SNR condition (i.e., $-20dB$).
The minimal SNR (for achieving the same SER) then grows to $-14dB$ and further to $-9dB$ as the spreading factor drops to 9 and 7, respectively.
The result demonstrates that the non-linear chirp achieves superior noise tolerance as the linear chirp does.

Since the LoRa symbol varies with the chirp's initial frequency offset, given a certain type of non-linear chirp, one may worry that the SER of this chirp may not be consistent across different LoRa symbols.
%and causes inconsistency in demodulating different symbols.
To validate this concern, we generate different chirp symbols by varying the initial frequency offset of a standard up-chirp. We then compare its symbol error rate with linear-chirps in the same SF settings.
As shown in Figure~\ref{subfig-nonlinear-vs-linear-noise-2}, the linear and non-linear chirps achieve very similar SER in all three SF settings.

%further illustrates the uniform SER distribution for non-linear chirps in the code space. Both verifies that non-linear chirps performs consistently with linear chirps, without any sacrifice on SNR gains for CSS modulation of LoRa. 

% Upon receiving massive encoded chirp symbols under various SFs, we first add Additive White Gaussian Noise (AWGN) manually for fine-grained SNR control. Then the SER trend of SNR can be derived in Figure~\ref{subfig-nonlinear-vs-linear-noise-1}, which demonstrates the consistent noise resilience between linear and non-linear chirps. For example, the SER keeps under 1\% for SF=11 for all kinds of chirps~\cite{LoSee}.
% Given the non-linear growth of frequency over time, one concern is that whether the SER can be varied with different encoded initial frequency. Figure~\ref{subfig-nonlinear-vs-linear-noise-2} further illustrates the uniform SER distribution for non-linear chirps in the code space. Both verifies that non-linear chirps performs consistently with linear chirps, without any sacrifice on SNR gains for CSS modulation of LoRa. 

\subsection{Power Consumption}
\label{subsec-design-4}

Next, we show that the non-linear chirp generation consumes the same order of power as the linear chirp generation does.
%In this section, we evaluate the power consumption of \ours, including the generation of baseband nonlinear chirp signal and the up-conversion to the radio frequency (RF).
% Existing approaches on chirp signal generation can be broadly divided into three schemes: $i)$: Direct analog frequency synthesizer; $ii)$: Direct digital frequency synthesizer; and $iii)$: Indirect frequency synthesizer). 
% The direct analog frequency synthesizer leverages a high-frequency clock to generate a high-frequency signal first, and then converts this signal into multiple signals with various frequencies using frequency divider and mixer.
% The direct digital frequency synthesizer 
We leverage Direct Digital Synthesis (DDS)~\cite{dds_tutorials}, a digital signal processing method to generate chirp signals. 
Compared to other analog frequency synthesis~\cite{analog_frequency} or voltage-controlled oscillator (VCO)~\cite{talla2017lora} based approaches, DDS is immune to both frequency and amplitude drifts and thus has been widely adopted for chirp signal generation in a radar system, e.g., frequency modulated continuous wave (FMCW) radars~\cite{dds_fmcw1, dds_fmcw2} and synthetic aperture radars (SAR)~\cite{dds_SRA1, dds_SRA2}. 

%Due to the advantage of accurate frequency control, fast dynamic frequency adjustment, and immune to frequency and amplitude drifts, DDS has been widely used for chirp signal generation in radar system, e.g., frequency modulated continuous wave (FMCW) radars~\cite{dds_fmcw1, dds_fmcw2} and synthetic aperture radars (SAR)~\cite{dds_SRA1, dds_SRA2}.

% from a reference frequency source by controlling the phase increment~\cite{dds_tutorials}. Due to the advantage of accurate frequency control, fast dynamic frequency adjustments, immune to frequency and amplitude drifts, DDS has been widely applied in various fields like frequency modulated continuous wave (FMCW) radars~\cite{dds_fmcw1, dds_fmcw2} and synthetic aperture radars (SAR)~\cite{dds_SRA1, dds_SRA2}.

DDS works as follows. It first generates a reference signal at a constant frequency $f_{clk}$, and stores the signal samples in a local buffer, called a phase-amplitude mapping-table. Let $L$ be the length of this mapping-table.
To generate a desired chirp signal, DDS then accesses the mapping-table following the equation defined below: 
%
\begin{equation}
\begin{split}
\label{eq:dds_frequency}
\phi_i=\sum\limits_{m=1}^{i}f_i=\sum\limits_{m=1}^{i}(f_{i-1}+K_i \times \frac{f_{clk}}{2^L})=\sum\limits_{m=1}^{i}\sum\limits_{j=1}^{m}K_i \times \frac{f_{clk}}{2^L}
\end{split}
\end{equation}
%
where $\phi_i$ and $f_i$ represent the phase and frequency of the $i^{th}$ sampling point of the chirp signal to be generated, respectively. $K_i$ is the slope of this chirp signal, describing how its frequency changes over time.
$K_i$ is a constant value for linear chirps. It varies over time for non-linear chirps.
The transmitter then retrieves these signal samples from the mapping-table and generates the chirp signal accordingly.

Figure~\ref{fig:dds} describes DDS's high-level operations.
To generate a linear chirp (Figure~\ref{fig:dds}(a)), the transmitter sets $K_i$ to a constant value (i.e., 1) and accesses the frequency samples at index (1, 2, 3, 4, ...). The phase samples are retrieved at index (1, 3, 6, 10, ...).
In contrast, to produce a non-linear chirp (Figure~\ref{fig:dds}(b)), $K_i$ varies over time, e.g., ($K_1$=1, $K_2$=2, $K_3$=4, $K_4$=8, ...). The frequency and phase index then changes to (1, 3, 7, 15, ...) and (1, 4, 11, 26, ...), respectively. 
%Finally, the corresponding amplitude is extracted from the pre-stored mapping table.

\vspace{1mm}
\noindent
\textbf{Validation.}  We prototype DDS on a Zynq-7000 FPGA~\cite{FPGA} and measure the power consumption of linear and non-linear chirp generation, respectively.
The FPGA board is equipped with an ultra low-power 12-bit ADC and a 256KB RAM.
The phase-amplitude mapping-table is generated by a 1~MHz clock signal. It stores $2^{12}$ sample points.
We then retrieve signal samples from this mapping table to generate chirps (bandwidth=125KHz, SF=7).
The sampling points of each chirp in total are 8192.
Our measurement study shows that the transmitter consumes the same order of power on generating the baseband of these two types of chirp signals: 315.6~$\mu W$ for non-linear chirps and 306.2~$\mu W$ for linear-chirps, respectively.
% The evaluation results show that the energy consumption of generating nonlinear chirp  signal and linear chirp signal is in the same order of magnitude, about 315.6~$\mu W$ and 306.2~$\mu W$, respectively. The difference of power consumption mainly comes from the difference of the frequency modulation slope $K_i$. 
The up-conversion of baseband to RF band (900~MHz) consumes around 40~mW~\cite{upconverter} for both chirps.
Hence the total power consumption (baseband+RF) of the DDS-based approach is similar to commercial LoRa nodes~\cite{LoRa_Transceiver}.


\begin{figure}[t]
    \centering
    \includegraphics[width=3.5in]{figures/non_linear_chirp.pdf}
    \vspace{-4mm}
    \caption{An illustration of DDS operation on generating the linear and non-linear chirps, respectively.}
    \label{fig:dds}
    \vspace{-4mm}
\end{figure}


%Moreover, the power consumption of baseband signal up-conversion to RF band (900~MHz) is 40~mW~\cite{upconverter}. Therefore, the power consumption of \ours is comparable with the commercial LoRa device~\cite{LoRa_Transceiver}.

% \subsection{SF-adaptive Collision Resolving}
% \label{subsec-design-5}

%\subsection{Noise and Interference Model}
%\label{subsec-noise-interference-model}

%Now radios can transmit data over these new logical channels created by nonlinear chirps. Whether these logical channels can keep low SNR/SIR requirements regarding to the noises from environment and the interference from other coexistent logical channels is still a question. Next, we first analyze the influence of environment noise. Then, we develop an interference model to depict the mutual constraint between two logical channels.

%\subsubsection{Environment Noise}
%\label{subsubsec-environment-noise}

%We assume the environment noise is white Gaussian noise. To analyze the influence of environment noise on \ours, we empirically study the symbol error rate (SER) of \ours under various SNR incurred by environment noise. Specifically, we use Monte Carlo simulation and compare both convex up-chirp (i.e., $f(x)=x^2$) and concave up-chirp (i.e., $f(x)=2x-x^2$) with LoRa linear chirp under three different SF settings (i.e., 7, 9, 11). For each scenario, various Additive White Gaussian Noise (AWGN) is added to transmitted shifted up-chirps to make different SNR. We manually align shifted up-chirp symbols to the corresponding baseline down-chirp for demodulation. For each scenario, we run 100,000 times to calculate the average SER.

%The results are shown in Figure~\ref{fig-environment-noise}. We can see that the SER-SNR relationship under different types (e.g., linear, convex, concave) of up-chirps with the same SF is quite similar. When SF is 7, to ensure SER is lower than 0.1\%, the SNR of the received signal should larger than about -7.5 dB. Similarly, when SF becomes 9 and 11, the SNR requirements are about -12.5 dB and -17.5 dB respectively, which can further tolerate the signal attenuation and multi-path interference in a long distance.
%Overall, \ours keeps the strong ability to resist environment noise as LoRa does. While using different types of nonlinear chirps (e.g., convex, concave), the demodulation is noise resilient. Thus, we have a large set of nonlinear functions to create new logical channels

%\subsubsection{Logical Channel Interference} 
%\label{subsubsec-logical-channel-interference}

%Regarding to Gaussian environment noise, there are countless polynomial coefficient combinations to construct various nonlinear chirps. However, whether different types of linear and nonlinear chirps can coexist with each other is another important aspect to maximize networking capacity by involving coexistent linear and nonlinear chirps as much as possible. 

%Given two chirp types, one is called \emph{reference signal} $C_r$ and the other is called \emph{interference signal} $C_i$, we use SIR model to indicate the influence of $C_i$ on $C_r$ demodulation.
%As shown in Figure~\ref{fig-SIR-definition}, the reference signal $C_r$ is a nonlinear up-chirp and the interference signal $C_i$ is a linear up-chirp. After we use dechirp process to demodulate a $C_r$ symbol (e.g., red solid curve), in FFT results, $p_r$ indicates the amplitude of the FFT bin that corresponding to the frequency shift used to modulate the $C_r$ symbol, and $p_i$ indicates the highest amplitude of the FFT bin among a series of FFT bins that are derived by multiplying the $C_i$ symbol (e.g., blue dashed line) with baseline $C_r$ down-chirp (e.g., red dashed curve).
%The $C_r$ symbol can be correctly demodulate if only if $p_r$ is higher than $p_i$. When $p_r$ equals to $p_i$, we define the corresponding SIR between $C_r$ and $C_i$ as a SIR threshold $SIR_{C_r}(C_i)$ which means $C_r$ can coexist with $C_i$ only if the SIR is larger than $SIR_{C_r}(C_i)$.

%Moreover, to accurately measure $SIR_{C_r}(C_i)$, we should further consider different overlapping patterns between $C_r$ symbol and $C_i$ symbol as shown in Figure~\ref{fig-overlap-pattern}. An overlapping pattern consists of two factors. First, $C_r$ (e.g., red solid curve) and $C_i$ (e.g., blue dashed line) may not synchronize with each other. The time gap $t_{gap}$ between $C_r$ and $C_i$ symbols can lead to different SIR thresholds. Second, the start frequency $f_0(C_i)$ of the overlapped $C_i$ symbols may vary so that lead different power density distribution along different frequencies after multiplying a nonlinear baseline down-chirp. Thus, the resulted SIR threshold varies.

%To accurately estimate the SIR threshold $SIR_{C_r}(C_i)$, we utilize Monte Carlo method to uniformly traverse the diversity of overlapping pattern as much as possible. Specifically, we gradually decrease SIR between $C_r$ and $C_i$ from -1 to -30. Give a SIR and the chirp types (e.g., SF, BW and polynomial coefficients) of $C_r$ and $C_i$, we randomly generate the start frequencies of the $C_r$ and $C_i$ symbols to construct different overlapping patterns. The reference baseline down-chirp symbol is aligned to the reference up-chirp manually. A symbol error appears when we fail to demodulate the $C_r$ symbol under this settings. We do not stop running the simulation until we observe 100 symbol errors. Then, SER is calculated as the ratio between 100 and the total rounds we have run. Finally, after getting a SIR below which the SER of the reference signal is higher than 1\%, we recognize the SIR as the SIR threshold. 

%\begin{figure}[t]
%    \includegraphics[width=0.5\textwidth]{figures/SIRheatmap.pdf}
%    \caption{SIR threshold heatmap of 30 chirp types. Each block indicates the SIR threshold of a reference signal (i.e., row mark) under an interference signal (i.e., column mark). The marks with a rectangle are LoRa linear chirps. With a darker color, the block corresponds to a lower SIR threshold.}
%    \label{fig-SIRheatmap}
%\end{figure}

%To understand SIR thresholds under different settings, we select five polynomial functions which include $x$, $x^2$, $1-(x-1)^2$, $x^4$ and $1-(x-1)^4$. We choose neither high-degree nonlinear functions (e.g., $x^5$) nor similar shaped nonlinear functions (e.g., $x^3$ and $x^4$). For high-degree nonlinear functions, their SIR threshold will be high regarding to the interference signals which hold the same function with different SFs due to their similar curve shapes. For similar shaped nonlinear functions, the SIR threshold will be high, too. The higher the SIR threshold is, the easier the collision happens. 
%Combining with 6 SF options, we have total 30 logical channels to calculate SIR threshold with each other. 

%The resulted SIR threshold heatmap is shown in Figure~\ref{fig-SIRheatmap}. We mark $x$ as \emph{linear}, $x^2$ as \emph{quadratic1}, $1-(x-1)^2$ as \emph{quadratic2}, $x^4$ as \emph{quartic1}, and $1-(x-1)^4$ as \emph{quartic2}. According to Figure~\ref{fig-SIRheatmap}, we have several observations as follows:

%(1) Let us compare the blocks in the bottom rows (i.e., logical channels with large SF) with the ones in the top rows (i.e., logical channels with small SF). We can see the color of the bottom part is deeper than the top part. This indicates that for both linear and nonlinear logical channels, large SF can improve the ability of interference resilience, but the cost is losing channel throughput.

%(2) Let us look at the blocks of three rows SF7-linear, SF7-quadratic1 and SF7-quartic1. We can see when interference signals have higher SFs, the SIR thresholds  of SF7-quartic1 are higher than that of SF7-linear and SF7-quadratic1. The similar phenomenon can be observed among linear, quadratic and quartic chips with the same SF. This verifies that for high-degree nonlinear functions, the logical channels created by different SFs can easily interfere with each other.

%(3) Let us compare the blocks in the left-bottom part with those in the right-top part. We can see the color of left-bottom part is deeper than that of right-top part which means the mutual interference between two logical channels is not symmetric. The more different the SFs are, the more asymmetric the SIR threshold is.

%(4) Let us focus on the blocks on the diagonal line of the heatmap. Each block indicates the SIR threshold under the interference from the same logical channel. For a linear logical channel, the resulted SIR threshold is not less than -2 dB (e.g., light yellow color), which means the only the strong signal can be demodulated, but the weak signal barely can be demodulated. In contrast, nonlinear logical channel can resist the self-interference with a lower SIR threshold (e.g., deep color). For quadratic chirps, when SF is 12, SIR threshold under self-interference is as low as -16 dB. This indicates that nonlinear logical channels are more resilient to self-interference that linear ones.

%(5) Let us compare the blocks of linear logical channels by separately taking quadratic chirps and quartic chirps as interference under the same SF. Taking the block pairs [(SF7-linear, SF7-quadratic1), (SF7-linear, SF7-quartic1)] and [(SF8-linear, SF8-quadratic1), (SF8-linear, SF8-quartic1)] as examples, we can see the blocks rendered by (SF7-linear, SF7-quadratic1) and (SF8-linear, SF8-quadratic1) have lighter color than (SF7-linear, SF7-quartic1) and (SF8-linear, SF8-quartic1), respectively. We notice that the shape of quadratic chirp is more similar with that of linear chirp than quartic chirp, this verifies that two logical channels can interfere each other easily when the shapes of their chirp functions are similar.

%\subsection{Logical Channel Selection}
%\label{subsec-logical-channel-selection}

%\begin{algorithm}[t]\footnotesize
%    \SetAlgoLined
%    \KwIn{A SIR threshold heatmap $SIR\_Heatmap$; a set of candidate logical channels $Candidate\_set$; the maximum average SIR threshold $SIR_T$.}
%    \KwOut{A set of logical channels $\ours\_set$}
%    Initialize $\ours\_set$ = \{ SF7-linear, ..., SF12-linear \}\;
%    \While{!isempty($Candidate\_set$)}{
%        $min\_SIR\_channel = NULL$ \;
%        $min\_SIR = 0$ \;
%        \ForAll{$channel \in Candidate\_set$}{ 
%          $mean\_SIR(channel) = \frac{\sum_{c\in{\ours\_set}}(SIR_{channel}(c) + SIR_{c}(channel)) + SIR_{channel}(channel)}{2|\ours\_Set|+1} $ \;
%        \If{$mean\_SIR(channel) < min\_SIR$}
%        {$min\_SIR = mean\_SIR(channel)$ \;
%        $min\_SIR\_channel = channel$ \;}
%        }
%        \If{$min\_SIR \geq SIR_T$} 
%        { break \;}
%        $\ours\_set = \ours\_set \cup \{mini\_SIR\_channel\}$  \;
%        $Candidate\_set = Candidate\_set \setminus \{mini\_SIR\_channel\}$ \;
%     }
%     \caption{Logical Channel Selection}\label{alg-ChirpOptionAlgorithm}
%    \end{algorithm}

%Given a set of available logical channel candidates and the SIR threshold between each pair of logical channels, our problem is to select a subset of these logical channels to optimize LoRaWAN capacity. When we add a new logical channel in LoRaWAN, the network capacity can be degraded only if there is a high probability that the transmissions using the new logical channel can collide with the transmissions using existing logical channels. According to our analysis in Section~\ref{subsec-noise-interference-model}, the interference resilience and channel capacity of different logical channels are very diverse. It is a difficulty problem to model the collisions by traverse all possible cases.

%Intuitively, we can utilize the average SIR threshold between a new logic channel and the existing logic channels as a metric to reflect the potential collisions. The higher the average SIR threshold is, more collisions probably happen. Then, we define a preconfigured maximum average SIR threshold which is use to judge whether a new logical channel should be added.

%As shown in Algorithm~\ref{alg-ChirpOptionAlgorithm}, we develop a greedy algorithm to iteratively select valid logical channels. Specifically, we initialize $\ours\_set$ as 6 linear chirps with SFs from 7 to 12. Given a set of logical channel candidates $Candidate\_set$, we repeatedly move the candidate with the minimum average SIR threshold with existing logical channels in $\ours\_set$ from $Candidate\_set$ to $\ours\_set$, until the minimum average SIR threshold is not less than  the preconfigured maximum average SIR threshold. The settings of the maximum average SIR threshold are empirically studied in Section~\ref{sec-evaluation}.

%-12.46, the average SIR threshold of LoRa's linear SF7 chirp in all possible overlapping scenarios with other LoRa linear chirps.

%After running the algorithm, there are 26 chirp options left in $\ours\_set$. Compared with all 30 pre-selected options, the algorithm excludes quartic1-SF7 ($x^4$-SF7), quartic1-SF8, quartic2-SF7 ($1-(x-1)^4$-SF7), and quartic2-SF8 chirps from the set.



==> CurvingLoRa NSDI 22/5System.tex <==
\section{CurvingLoRa PHY-Layer}
\label{sec-system}
The above section shows a set of desirable properties of non-linear chirps, in this section, we describe the PHY-layer design on non-linear chirp modulation (\S\ref{subsec-system-1}), demodulation (\S\ref{subsec-system-2}), and the frame format for packet detection (\S\ref{subsec-system-3}).
%First, we illustrate the format of \ours frame. Second, we discuss the nonlinear functions to build \ours logic channels to enlarge LoRaWAN capacity. Third, we introduce the prototype hardwares to implement \ours radio and gateway. At last, we depict the experiment environment of our outdoor and indoor deployment.


\subsection{Modulation}
\label{subsec-system-1}


Similar to the standard linear chirp modulation in LoRa, \ours defines a base non-linear chirp and modulates it by varying its initial frequency offset. 

\noindent \textbf{Base non-linear chirp generation}. We define a base non-linear chirp as a monotonic curve growing from $(0, -\frac{BW}{2})$ to $(\frac{2^{SF}}{BW}, \frac{BW}{2})$, where the coordinate $(x,y)$ represents the (time, frequency) boundary of this chirp.
$SF$ and $BW$ denote the spreading factor and bandwidth, respectively.
Since a monotone nonlinear function can be approximated by the sum of a set of polynomial functions in time-frequency domain, the base non-linear chirp thus can be represents as:
\begin{equation}
\label{equ-nonlinear-baseline-up-chirp} 
    \begin{split}
    f_c(t) &= \sum^{n}_{i=0}k_it^i, t \in [0,\frac{2^{SF}}{BW}], f_c(t) \in [-\frac{BW}{2},\frac{BW}{2}] \\
    \end{split}
\end{equation}
where $k_i, i\in[0,n]$ are a set of coefficients to fit the non-linear curve into the range of symbol time and bandwidth. 
Notice that for a linear chirp, all these coefficients are zero except for $k_0=-\frac{BW}{2}$ and $k_1=\frac{BW^2}{2^{SF}}$.

To facilitate the coefficient configuration in different $BW$ and $SF$ settings, we further design a polynomial chirp function in a unified space ($[0,1]_x\times[0,1]_{f(x)}$) as follow:
\begin{equation} 
\label{equ-unified-space-function}
    \begin{split}
    f(x) &= \sum^{n}_{i=0}a_ix^i, x \in [0,1], f(x) \in [0,1] \\
    \end{split}
\end{equation} 
where $a_i,i\in[0,n]$ is the $i^{th}$ coefficient. The relationship between the coefficient defined in the unified space and that defined in the time-frequency domain (i.e., $k_i$ in Equation~\ref{equ-nonlinear-baseline-up-chirp}) can be represented as follows:
%We then transform $a_i$ defined in the unified space into the time-frequency domain coefficients $k_i$ defined in Equation~\ref{equ-nonlinear-baseline-up-chirp} as follow:
\begin{equation}
	\label{equ-coefficient-mapping}
	\begin{split}
		k_0 = BW \times a_0-\frac{BW}{2},\;
		k_i = \frac{BW^{i+1}}{2^{SF\times i}}a_i, i\in[1,n]
	\end{split}
\end{equation} 

Given $BW$ and $SF$, we can compute the coefficient $k_i$ for each polynomial term defined in Equation~\ref{equ-nonlinear-baseline-up-chirp} and generate the base up-chirp accordingly.
The down-chirp can be generated by conjugating the base up-chirp.

\noindent \textbf{Base non-linear chirp modulation}. Once we have a base non-linear chirp, the transmitter then varies the initial frequency offset of this base chirp to modulate data:
\begin{equation} 
\label{equ-shifted-nonlinear-chirps}
    \begin{aligned}
        h(t) &=  
    e^{j 2 \pi (f_0+f_c(t)) t} 
    \end{aligned}
\end{equation}
where $f_0$ is the initial frequency offset of this chirp.
In essence, given the same $BW$ and $SF$ configurations, \ours achieves the same link throughput with the standard linear-chirp based LoRa.

\noindent \textbf{Modulation knobs}. By using different polynomial functions defined in the unified space (e.g., $f(x)=x$, $f(x)=x^2$ and $f(x)=2x-x^2$), the transmitter can easily build different base chirps.
Figure~\ref{fig-unified-symbol-modulation} shows a convex and a concave non-linear chirp produced by two different polynomial functions.
These different polynomial functions provide us another knob to boost the capacity of concurrent LoRa transmissions.
To understand the rationale behind this, let's consider a case where two LoRa transmissions (i.e., $S_A$ and $S_B$) are happenly well aligned at the receiver.
Let $S_R$ be their superposition.

% \begin{figure}[t]
%     \includegraphics[width=0.4\textwidth]{figures/LoRaDechirp3.pdf}
%     \caption{The correct demodulation of a reference symbol given a interference symbol.}
%     \label{fig-linear-and-nonlinear}	
% \end{figure}

\begin{figure}[t]
    \centering
    \subfigure[Linear up-chirp]{ 
        \includegraphics[width=0.33\columnwidth]{nsdi_pdf/mapping12.pdf}
        \label{subfig-linear-mapping}
        }
    \hspace{-0.06\columnwidth}
    \subfigure[Convex up-chirp]{
        \includegraphics[width=0.33\columnwidth]{nsdi_pdf/mapping22.pdf}
        \label{subfig-convex-mapping}
        }
     \hspace{-0.06\columnwidth}
    \subfigure[Concave up-chirp]{
        \includegraphics[width=0.33\columnwidth]{nsdi_pdf/mapping32.pdf}
        \label{subfig-concave-mapping}
        }
        % \vspace{-4mm}
    \caption{An illustration of linear and non-linear chirps with the corresponding function parameters.
    % Converting the curve defined by a linear/nonlinear function $f(x)$ in $[0,1]_x\times[0,1]_{f(x)}$ to baseline up-chirp in time-frequency domain $[0,\frac{2^{SF}}{BW}]\times[-\frac{BW}{2},\frac{BW}{2}]_f$. (a) Linear up-chirp, (b) nonlinear convex up-chirp (i.e., $f(x) = x^2$), (c) nonlinear concave up-chirp (i.e., $f(x) = 2x - x^2$).
    }
    \label{fig-unified-symbol-modulation}
    \vspace{-4mm}
\end{figure}

\begin{figure}[t]
    \centering
    \subfigure[L. meets L.]{ 
        \includegraphics[width=0.30\columnwidth]{figs/linear_linear.pdf}
        \label{subfig-knobs-1}
        }
    % \hfill
    \subfigure[NL. meets NL.]{
        \includegraphics[width=0.30\columnwidth]{figs/nonlinear_nonlinear.pdf}
        \label{subfig-knobs-2}
        }
    % \hfill
    \subfigure[NL. meets L.]{
        \includegraphics[width=0.30\columnwidth]{figs/linear_nonlinear.pdf}
        \label{subfig-knobs-3}       
        }
        % \vspace{-4mm}
    \caption{An illustration of symbol collisions.
    {\normalfont
    (a): A linear chirp (L.) collides with another linear chirp. (b): A non-linear (NL.) chirp collides with another non-linear chirp. (c): A non-linear chirp collides with a linear chirp.}}
    \vspace{-4mm}
\label{fig-knobs}
\end{figure}

\noindent $	\bullet$ \textbf{Case one}: when both $S_A$ and $S_B$ are linear chirps, we are expected to see two separate energy peaks on FFT bins (shown in Figure~\ref{subfig-knobs-1}). In this case, all existing parallel decoding approaches~\cite{mLoRa,oct,xia2019ftrack,colora,tong_combating_2020,xu_fliplora_2020,eletreby2017empowering,hu2020sclora} fail to disambiguate the collision symbols as these two well-aligned symbols exhibit similar FFT peaks. 
    
\noindent $	\bullet$ \textbf{Case two}: when both $S_A$ and $S_B$ are non-linear chirps (i.e., generated by two different polynomial functions), the receiver can decode each symbol from their collision as follows.
The receiver first multiplies $S_R$ with the conjugate of $S_A$. As a result, the energy of $S_B$ will be spread over multiple FFT bins, whereas the energy of $S_A$ will concentrate on a single, isolated FFT bin, as shown in Figure~\ref{subfig-knobs-2}.
%We are expected to see a single energy peak plus a cluster of weak energy peaks on FFT bins. 
%This single, isolated energy peak is produced by $S_A$ and is significantly stronger than every single peak within another cluster of energy peaks. 
The receiver can easily pick up this energy peak and decode $S_A$. $S_B$ can be decoded similarly by replacing the down-chirp with the conjugate of $S_B$.

\noindent $	\bullet$ \textbf{Case three}: when one of the LoRa symbols is based on linear chirp and another is based on non-linear chirp, similar to case two, the receiver can alternate between different down-chirps to decode each of them accordingly, as shown in Figure~\ref{subfig-knobs-3}.


We have three takeaways from the above analysis: $i)$ the transmitters can use different types of non-linear chirps as an orthogonal approach to boost the concurrency of LoRa transmissions.
$ii)$ the non-linear chirp based LoRa nodes can  co-exist with those linear-chirp based legacy LoRa nodes. 
$iii)$ the adoption of different non-linear chirps also facilitates the demodulation of well-aligned collision symbols.
% In contrast, none of the existing linear-chirp based demodulation approaches is able to handle it.

%In such case, all existing parallel decoding approaches~\cite{} based on linear-chirp fail to work as they cannot differentiate two FFT peaks after dechirping, as shown in Figure~\ref{}.
%In contrast, \ours can reliably demodulate these two collision chirps by applying different conjugate down-chirp in dechirping process.
%As shown in Figure~\ref{}, the multiplication of

% Figure~\ref{fig-unified-symbol-modulation}, the coefficients of baseline linear (e.g., Figure~\ref{subfig-linear-mapping}), convex(e.g., Figure~\ref{subfig-convex-mapping}) and concave (e.g., Figure~\ref{subfig-concave-mapping}) up-chirps can be converted from the corresponding functions (e.g., $f(x)=x$, $f(x)=x^2$ and $f(x)=2x-x^2$) in the unified space $[0,1]_x\times[0,1]_{f(x)}$.

% We adopt the parameters $BW$ and $SF$ to constrain the range of a nonlinear chirp in time-frequency domain. 
% As shown in Figure~\ref{fig-unified-symbol-modulation}, baseline nonlinear up-chirps are monotone line/curves which start at $(0, -\frac{BW}{2})$ and end at $(\frac{2^{SF}}{BW}, \frac{BW}{2})$.
% Since a monotone nonlinear function can be approximated by the sum of a set of polynomial functions, in time-frequency domain, its baseline up-chirp can be calculated as follow:
% \begin{equation}
% \label{equ-nonlinear-baseline-up-chirp} 
%     \begin{split}
%     f_c(t) &= \sum^{n}_{i=0}k_it^i, t \in [0,\frac{2^{SF}}{BW}], f_c(t) \in [-\frac{BW}{2},\frac{BW}{2}] \\
%     \end{split}
% \end{equation}
% where $k_i, i\in[0,n]$ are a set of coefficients which make the curve to fit the ranges of time and frequency. For linear chirp, besides $k_0=-\frac{BW}{2}$ and $k_1=\frac{BW^2}{2^{SF}}$, all other coefficients are 0.

% Given baseline nonlinear up-chirp in time-frequency domain $[0,\frac{2^{SF}}{BW}]\times[-\frac{BW}{2},\frac{BW}{2}]_f$, We modulate data by modifying the start frequency of baseline nonlinear up-chirp as LoRa does with baseline linear up-chirp. A shifted nonlinear chirp based symbol is calculated as follow:
% \begin{equation} 
% \label{equ-shifted-nonlinear-chirps}
%     \begin{aligned}
%         h(t) &=  
%     e^{j 2 \pi (f_0+f_c(t)) t} 
%     \end{aligned}
% \end{equation}
% where $f_0$ is the start frequency to represent SF bits data. In this way, given the same $BW$ and $SF$ settings, the channel throughput is the same between \ours and LoRa.

% To easily adjust the coefficients $k_i$ of baseline nonlinear chirp under different settings of $BW$ and $SF$, we first design polynomial chirp function in a unified space defined as $[0,1]_x\times[0,1]_{f(x)}$ as follow:
% \begin{equation} 
% \label{equ-unified-space-function}
%     \begin{split}
%     f(x) &= \sum^{n}_{i=0}a_ix^i, x \in [0,1], f(x) \in [0,1] \\
%     \end{split}
% \end{equation} 
% where $a_i,i\in[0,n]$ are the coefficients. Then we convert a unified space coefficients $a_i$ to the time-frequency domain coefficients $k_i$ defined in Equation~\ref{equ-nonlinear-baseline-up-chirp} as follow:
% \begin{equation}
% 	\label{equ-coefficient-mapping}
% 	\begin{split}
% 		k_0 &= BW \times a_0-\frac{BW}{2} \\
% 		k_i &= \frac{BW^{i+1}}{2^{SF\times i}}a_i, i\in[1,n]
% 	\end{split}
% \end{equation} 
% As shown in Figure~\ref{fig-unified-symbol-modulation}, the coefficients of baseline linear (e.g., Figure~\ref{subfig-linear-mapping}), convex(e.g., Figure~\ref{subfig-convex-mapping}) and concave (e.g., Figure~\ref{subfig-concave-mapping}) up-chirps can be converted from the corresponding functions (e.g., $f(x)=x$, $f(x)=x^2$ and $f(x)=2x-x^2$) in the unified space $[0,1]_x\times[0,1]_{f(x)}$.

% Our unified symbol modulation consists of three steps. First, we design a nonlinear function in the unified space. Then, we convert the nonlinear function to the baseline nonlinear up-chirp and down-chirp. At last, we generate shifted nonlinear up-chirps to modulate data.

\subsection{Demodulation}
\label{subsec-system-2}

\begin{figure}[t]
    \centering
    \subfigure[with STO and CFO] {
    \includegraphics[width=0.29\columnwidth]{figs/offset_1.pdf}
    	\label{subfig-symbol-alignment}
    }
    % \hfill
    \subfigure[with CFO]{ 
    %\centering
    \includegraphics[width=0.29\columnwidth]{figs/offset_2.pdf}
        \label{subfig-fixCFO1}
    }
    %\hspace{2em}
    % \hfill
    \subfigure[with STO and CFO]{
    %\centering
        \includegraphics[width=0.29\columnwidth]{figs/offset_3.pdf}
        \label{subfig-fixCFO2}
    }
    % \vspace{-4mm}
    \caption{The influence of symbol time offset (STO) and carrier frequency offset (CFO) on demodulation. 
    {\normalfont
    (a) both STO and CFO move the energy peak of a linear chirp from its desired FFT bin.
    (b) CFO moves the energy peak of a non-linear chirp from its desired FFT bin. 
    (c) STO spreads the power of a non-linear chirp into multiple FFT bins.}}
    \vspace{-4mm}
     \label{fig-fixCFO}
\end{figure}


Similar to linear chirp demodulation, the receiver operates dechirp to demodulate non-linear chirps.
%\begin{align}
%&e^{j 2 \pi (f_0+f_c(t+t_{gap})) t}*e^{-j 2 \pi f_c(t) t}=e^{j 2 \pi F(t)t}\label{equ-dechirp}
%\end{align}
%where $t_{gap}$ denotes the symbol offset between the targeting chirp symbol and the observing window. The spectral energy of this chirp symbol is either focused on a specific frequency point (when $t_{gap}$=0) or spread into multiple frequency points (when $t_{gap}\neq$0).



% For linear chirps (e.g., $f_c(t)=k_1t+k_0$) in Equation~\eqref{equ-unified-space-function}, the dechirp can always focus the spectral energy at a single tone for any $t_{gap}$, whose constant frequency bin $f_0+k_1t_{gap}$ in Equation~\ref{equ-dechirp-linear} corresponds to the decoded data. 
% However, the spectral energy can be spread out for an misaligned non-linear chirp symbol (e.g., $t_{gap}\neq0$) while being focused for an aligned one (e.g., $t_{gap}=0$). Take the polynomial functions (\S\ref{subsec-system-1}): $quadratic1$---$f(t) = t^2$ as an example,  
% Equation~\ref{equ-dechirp-nonlinear} shows the time-varying frequency bins $F(t)=f_0+k_2t^2_{gap}+2k_2t_{gap}\times{t}$, which spreads the spectral energy linearly.
% \begin{align}
% % F(t)=f_0+f_c(t+t_{gap})-f_c(t)\nonumber\\
%  F(t)&=f_0+k_1(t+t_{gap})+k_0-(k_1t+k_0)=f_0+k_1t_{gap}\label{equ-dechirp-linear}\\
%  F(t)&=f_0+k_2(t+t_{gap})^2+k_0-(k_2t^2+k_0)\nonumber\\
% & =f_0+k_2t^2_{gap}+2k_2t_{gap}\times {t}\label{equ-dechirp-nonlinear}
% \end{align}

% Give different non-linear functions in Equation~\ref{equ-nonlinear-baseline-up-chirp}, the spectral energy can be spread out in a corresponding polynomial format, which determines the symbol error rate under various SIRs and SNRs in collisions (\S\ref{sec-evaluation}).


\noindent \textbf{Accounting for the Misalignment.} 
Symbol alignment is critical to the demodulation performance, particularly for non-linear chirp demodulation, as the misalignment will spread the spectrum power of a chirp symbol into multiple frequency points, which fails the demodulation.
%The receiver thus cannot reliably demodulate this symbol.
% In addition to symbol time offset (STO), the carrier frequency offset (STO) also introduces misalignment between chirp symbol and the down-chirp in the current observing window.
While this misalignment, in theory, is only caused by the symbol time offset (STO) between the incident chirp symbol and the down-chirp, in practice, it is also affected by the carrier frequency offset (CFO) caused by clock offset.


In linear chirp demodulation, the dechirp converges the spectrum power of each linear chirp symbol to a specific frequency point.
The existence of STO and CFO both renders the energy peak merely deviates from its desired position in FFT bins.
After the dechirp, the receiver can thus leverage the preamble to estimate such frequency shift and then correct the symbol by applying the estimated frequency shift to the energy peak.
However, such a post-processing approach cannot be directly applied to non-linear chirp, as the existence of STO will instead spread the spectrum energy into multiple FFT bins.
Hence the receiver has to align the chirp symbol with the down-chirp and compensate for the CFO before operating dechirp on each non-linear chirp symbol.



% To ensure $f_c(t+t_{gap})-f_c(t))$ for successful demodulation of non-linear chirps, the key point is to resolve the misalignment issue induced by Symbol Time Offset (STO) and Carrier Frequency Offset (CFO). In linear chirp demodulation, both STO and CFO behave consistently and can be easily mitigated by comparing the pre-defined preamble and decoded preamble firstly and subtracting them for the decoded payloads directly. However, chirp symbol synchronization and offset calibration have to be resolved at the beginning for non-linear chirps, which can not be recovered from the spreading energy peaks once misaligned.




To better understand this issue, we take Figure~\ref{fig-fixCFO} as an example, where the receiver demodulates the linear chirp and non-linear chirp, respectively.
To align the incoming linear chirp shown in Figure~\ref{fig-fixCFO}(a), the LoRa receiver simply operates multiplication on these two chirps.
Due to the symbol time offset, the resulting FFT peak will be shifted from its desired bin by the amount of $\Delta_{STO}$.
%By leveraging the preamble in LoRa header, the receiver can easily figure out the misaligned interval by observing the shifting of FFT peak in the frequency domain and then synchronizes each incoming chirp with the down-chirp for reliable decoding.
CFO leads to an extra shift of the FFT peak $\Delta_{CFO}$.
By leveraging the preamble in the LoRa header, the receiver can easily estimate $\Delta_{CFO}$+$\Delta_{STO}$ and offset their impact on the energy peak.
In contrast, the multiplication of two misaligned non-linear chirps (shown in Figure~\ref{fig-fixCFO}(b)) spreads the spectrum energy into multiple FFT bins, as shown in Figure~\ref{fig-fixCFO}(b).
The existence of CFO further shift these FFT peaks and complicate the symbol alignment, as shown in Figure~\ref{fig-fixCFO}(c).
% Therefore, it is difficult to pick up one FFT peak from this cluster of energy peaks as a reliable reference to estimate the misaligned interval. 
% The existence of CFO will shift this cluster and complicate the symbol alignment further.

%\textbf{Takeaway:} The accurate alignment of chirp symbols is required to capture the potential gains of non-linear chirps. However, it can be computation exhausted to do the sample-by-sample search with the non-linear chirp based preamble. 

In \ours, we put a pair of conjugate chirps---a standard linear up-chirp followed by a standard linear down-chirp---as the pilot symbols of a LoRa packet to estimate the STO and CFO.
Suppose these two linear chirps
are well aligned with their conjugate counterpart in dechirping
process, respectively. 
The resulting two FFT peaks are supposed
to be superimposed at the same FFT bin in the absence of CFO.
On the contrary, the existence of $STO$ and $CFO$ will shift these two FFT peaks by the amount of $\Delta_{CFO}+\Delta_{STO}$ and $-(\Delta_{CFO}+\Delta_{STO})$ from their desired position.
The receiver then estimates the STO and CFO using the similar method as in NScale~\cite{tong_combating_2020} and offsets the symbol misalignment and carrier frequency offset accordingly.
It then operates dechirp on the corrected symbols to demodulate each symbol.



% \ours incorporates the linear chirps as the preamble to leverage its offset-agnostic energy focusing effect for packet alignment. Thus, the demodulation of non-linear chirp-based payloads can fully exploited the SNR and SIR gains in collisions.
% Specifically, a pair of conjugate linear chirps---a standard up-chirp followed by a standard down-chirp--- are designed as the pilot symbols of a LoRa packet. 
% Similar in Figure~\ref{subfig-fixCFO2}, the spectral energy of linear chirps will be shifted by amount of $b_{CFO}$ and $-b_{CFO}$ oppositely from their desired bin in the presence of CFO, but in a format of two FFT peaks. Thus, we can first leverage these opposite changes to remove CFO and then mitigate the pure STO by computing the symbol shift $b_{LoRa}(t_{gap})$ of linear chirp-based preamble in Figure~\ref{subfig-symbol-alignment}~\cite{colora,tong_combating_2020}.
% Now let us consider a more practical scenario where these two chirps are misaligned with their conjugate counterpart in dechirping process.
% In this case, we are expected to see two clusters of energy peaks in FFT bins, with each cluster corresponding to an individual non-linear chirp.
% In particular, these two clusters of energy peaks are symmetric to each other with an equal spacing ($b_{CFO}$) to their desired bin.
% This observation motivate us to take a sliding window-based approach to align these two pilot symbols with their respective conjugate counterpart sample by sample until each individual groups of FFT peaks are superimposed together.
% The CFO can be estimated accordingly by counting the spacing between two symmetric, superimposed FFT peaks.

% \noindent \textbf{Expediting symbol alignment}. 
% In practice, sample-by-sample search however is computationally intensive. 
% We thus develop a heuristic algorithm to expedite the frame alignment. 
% This heuristic is based on an observation that the FFT bin shift $b_{CFO}$ usually falls into a narrow range (detailed in Section~\ref{sec-implementation}).
% Without loss of generality, we define an empirical threshold $\delta$ to bound the range of $b_{CFO}$ as $[0, \delta] \cup [len-\delta, len]$, where $len$ is the number of FFT bins within a chirp symbol. \textcolor{red}{|}

% --------------------

% In \ours, we define an empirical threshold $\delta$ to bound the range of $b_{CFO}$ as $[0, \delta] \cup [len-\delta, len]$, where $len$ is the number of FFT bins within a symbol. 
% As shown in Algorithm~\ref{alg-CFOAlgorithm}, we use the start and end sample index $Pos_{init}$ and $Pos_{end}$ to indicate the search range of synchronization time offset $\Delta$. If the peak FFT bin $peak_1$ of the up-chirp symbol does not fall into the range after dechirp, we quickly increase the next sample index to get rid of the useless sample-by-sample search. Otherwise, we do not stop searching sample-by-sample until $peak_1$ and $peak_2$ (i.e., the peak FFT bin of the down-chirp symbol) are the same. Then, we accordingly calculate the $\Delta$ and $b_{CFO}$ which can ensure the accurate demodulation for the shifted up-chirp symbols in the same \ours packet.



% In \ours, given a symbol modulated by shifted nonlinear up-chirp $h(t)$ shown in Equation~\ref{equ-shifted-nonlinear-chirps}, we align the symbol to the conjugate baseline nonlinear down-chirp $e^{-j 2\pi f_c(t) t}$ and multiply them together to extract the start frequency $f_0$ by using FFT for symbol demodulation. For simplicity, we call this calculation process as \emph{dechirp}.
% For \ours gateway, the most important part of symbol demodulation is to synchronize the time between received symbols and local baseline down-chips.
% With nonlinear functions, however, the symbol misalignment cannot be simply calibrated as LoRa does. In LoRa, as shown in Figure~\ref{subfig-symbol-alignment}, given a baseline linear up-chirp (e.g., red solid line), if the misalignment interval is $\Delta$ between it and a baseline linear down-chirp (e.g., red dashed line), a single peak appears after dechirp. And its FFT bin offset $b_{LoRa}(\Delta)$ is proportional to $\Delta$ which can be accordingly estimated. In contrast, given a baseline nonlinear up-chirp (e.g., green solid curve) and a baseline nonlinear down-chirp (e.g., green dashed curve) with the same $\Delta$, after dechirp the total energy is scattered at multiple FFT bins (e.g, $b_{Curv}(\Delta \cdot t)$) which make $\Delta$ hard to be estimated. Moreover, as shown in Figure~\ref{subfig-fixCFO1}, due to the imperfect radio crystal, there is an unknown Central Frequency Offset (CFO) between received symbols (e.g., red solid curves) and standard baseline up-chirp and down-chirp (e.g., green dashed curves). Even when symbols are synchronized, a FFT bin offset of the single peak appears after dechirp so that misleads the symbol demodulation.

% \begin{algorithm}[t]\footnotesize
%     \SetAlgoLined
%     \KwIn{Received a pair of up-chirp and down-chirp symbols $h(t)$; the start and end sample index of the search range $Pos_{init}$ and $Pos_{end}$; total FFT bins of a symbol $len$; $b_{CFO}$ threshold $\delta$.}
%     \KwOut{Time offset $\Delta$; FFT bin $b_{CFO}$}
%     $h^*(t)$ = conjugate([standard baseline up-chirp + down-chirp])\;
%     \For{i=$Pos_{init}$;i<$Pos_{end}$;i++}{
%      	$H(t) = h(t+i)h^*(t)$ \;
%      	$peak_1$ = bin\_index(max(FFT(the up-chirp in $H(t)$]))) \;
%      	$peak_2$ = bin\_index(max(FFT(the down-chirp in $H(t)$))) \;
%      	\eIf{$peak_1<\delta$ or $len-peak_1<\delta$}{
%          \If{$peak_1 == peak_2$} { $\Delta = i - Pos_{init}$\;
%               $b_{CFO}$ = bin\_index(max(FFT($H(t)$)))\;
%               break \; }
%              %{111 \;}
%              }
%         { i= i+bin\_to\_sample(min($peak_1-\delta, len - \delta - peak_1$))-1 \;}
        
%      }
%     \caption{Symbol Alignment and CFO Estimation}
%     \label{alg-CFOAlgorithm}
% \end{algorithm}

% To achieve accurate symbol alignment and mitigate CFO, we utilize a pair of baseline up-chirp and down-chirp (e.g., red solid curves in Figure~\ref{subfig-fixCFO1}) embedded into \ours packet (Section~\ref{sec-implementation}). We have two observations. First, as shown in Figure~\ref{subfig-fixCFO1}, when symbols are synchronized, after dechirp, two peaks, derived from the up-chirp and down-chirp, will be superposed with each other at FFT bin $b_{CFO}$. Second, if symbols are not synchronized, as shown in Figure~\ref{subfig-fixCFO2}, we observe that after dechirp, the scattered FFT bins of the up-chirp and down-chirp will symmetrically distributed regarding to FFT bin $b_{CFO}$. Based on these two observation, to align symbols and estimate CFO, an intuitive method is to move the pair of standard down-chirp and up-chirp (e.g., green dashed curves) sample by sample until the respective maximum amplitude FFT bins of the up-chirp and down-chirp symbols  (e.g., red solid curves) are superposed.

% Sample-by-sample search, however, is computation exhausted so that degrades the demodulation efficiency. We further develop a heuristic algorithm to accelerate the search speed. Given the symbol The basic observation is that $b_{CFO}$ usually falls into a narrow range (Section~\ref{sec-implementation}). We can use an empirical threshold $\delta$ to bound the range of $b_{CFO}$ as $[0, \delta] \cup [len-\delta, len]$, where $len$ is the total FFT bins of a symbol. As shown in Algorithm~\ref{alg-CFOAlgorithm}, we use the start and end sample index $Pos_{init}$ and $Pos_{end}$ to indicate the search range of synchronization time offset $\Delta$. If the peak FFT bin $peak_1$ of the up-chirp symbol does not fall into the range after dechirp, we quickly increase the next sample index to get rid of the useless sample-by-sample search. Otherwise, we do not stop searching sample-by-sample until $peak_1$ and $peak_2$ (i.e., the peak FFT bin of the down-chirp symbol) are the same. Then, we accordingly calculate the $\Delta$ and $b_{CFO}$ which can ensure the accurate demodulation for the shifted up-chirp symbols in the same \ours packet.

% \begin{figure}[t]
%     \centerline{
%     \begin{minipage}[t]{0.24\textwidth}
%     \centering
%     \includegraphics[width=1\textwidth]{figures/LoRaDechirp3.pdf}
%     \caption{The correct demodulation of a reference symbol given a interference symbol.}
%     \label{fig-SIR-definition}	
%     \end{minipage}
%     % \hfill
%     \begin{minipage}[t]{0.24\textwidth}
%     \centering
%     \includegraphics[width=1\textwidth]{figures/overlapping.pdf}
%     \caption{The different overlapping patterns $t_{gap}$ derive different SIR threshold.}
%     \label{fig-overlap-pattern}	
%     \end{minipage}
%     }
% \end{figure}

\subsection{Frame Format}
\label{subsec-system-3}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/preamble.png}
    \vspace{-4mm}
    \caption{Packet format of \ours.}
    \label{fig-frame-format}
    \vspace{-4mm}
\end{figure}

% \begin{figure}[t]
%     \centerline{
%     \subfigure[SF=8] {
%     \includegraphics[width=0.33\columnwidth]{figs/sir2map_fs125k_SF8_preamble.png}
%     \label{subfig-preamble-linear-nonlinear-1}	
%     }
%     % \hfill
%     \subfigure[SF=10] {
%     \includegraphics[width=0.33\columnwidth]{figs/sir2map_fs125k_SF10_preamble.png}
%     \label{subfig-preamble-linear-nonlinear-2}	
%     }
%     % \hfill
%     \subfigure[SF=12] {
%     \includegraphics[width=0.33\columnwidth]{figs/sir2map_fs125k_SF12_preamble.png}
%     \label{subfig-preamble-linear-nonlinear-3}	
%     }
%     }\caption{Non-linear chirps collide with linear ones.\textcolor{red}{consider to move it to experiment.}}
%     \label{fig-preamble-linear-nonlinear}
% \end{figure}
A typical LoRa packet comprises multiple preamble symbols, 2 mandatory sync word symbols, 2.25 Start Frame Delimiter (SFD) symbols followed by a variable number of payload symbols~\cite{liando2019known,tong_combating_2020}.
Following the standard LoRa packet format, we encode the sync word symbols and payloads with non-linear chirps while retaining the linear chirps in preambles and SFDs, shown in Figure~\ref{fig-frame-format}.
The preamble contains 8 identical linear up-chirps for packet detection and alignment, followed by 2 non-linear chirps of sync word for configuration recognition of payloads.
The SFD consists of 2.25 standard down-chirps while the payload contains multiple chirp symbols with configurable length and chirp type. 
As mentioned in $\S$\ref{subsec-system-2}, a pair of up-chirp and down-chirp (i.e., pilot symbols) is needed to facilitate the symbol alignment.
Instead of putting an extra pair of such pilot symbols on the LoRa packet, we reuse the last linear up-chirp symbol in the LoRa preamble and the first linear down-chirp symbol of SFD as the pilots.
The use of linear chirp-based preamble may introduce the following two types of collisions:

\noindent \textbf{$\bullet$} Linear chirps collide with non-linear chirps when the preamble of one packet happenly aligns with the payload of another packet. In this case, the receiver can still leverage the energy scattering and converging effect to detect the preamble and further demodulate each individual signal (\S\ref{subsec-system-1}).

\noindent \textbf{$\bullet$} Linear chirps collide with linear chirps when the preamble of one packet happenly aligns with the preamble of another packet. In practice, however, this case rarely happens as the preamble contains only eight symbols, whereas the payload may last for hundreds of symbols~\cite{colora,tong_combating_2020}.


% One may concern that the use of linear chirp-based preamble may undermine the demodulation of collided symbols.
% To verify this concern, we measure the impact of the introduced preamble, especially in collisions, we conduct experiments to analyze the SIR threshold for collisions with different types of chirps, as Figure~\ref{fig-nonlinear-vs-linear-sir} does. 
% And collisions can occur between the linear preamble and the non-linear payloads, either of which can be the weak signals.
% Illustrated in Figure~\ref{fig-preamble-linear-nonlinear}, the weak linear preamble can collide with the strong non-linear payloads in two packets, of which the SIR threshold (e.g., blue) is far below the one for payload collisions (e.g., dark grey).
% The SIR threshold keeps lower than the payload collisions when the weak non-linear payloads collide with the strong linear preamble, across SF=8,10,12.
% Evaluation results demonstrate that the linear chirp-based preamble detection can guarantee the accurate packet alignment while not limiting the SIR gains for demodulation of payloads for non-linear chirps.
% As for collisions between two linear preamble, on one hand, it has little chance to happen for a long packets~\cite{colora,tong_combating_2020}, in which an 8-symbol preamble can be followed by a 100-symbol payload. 
% On the other hand, by correlating the packet with the pre-defined 8-symbol preamble for detection and alignment, the achieves SNR and SIR threshold is far below the payload demodulation.
% We further evaluation the effectiveness of our packet detection and alignment in our indoor and outdoor test-beds ($\S$\ref{sec-evaluation}).


% \subsection{Non-linear chirp Candidates}
% \label{subsec-system-4}
% \cl{not sure if it should be removed? Or we can discuss the difference between various types of non-linear chirps}

% \textcolor{red}{I think for now, we can remove this part. May discuss in length on the evaluation part.}

% As we discussed the characteristics of linear and nonlinear logical channels in Section~\ref{subsec-noise-interference-model}, we empirically select five polynomial functions which include $x$, $x^2$, $1-(x-1)^2$, $x^4$ and $1-(x-1)^4$, the same as we have studied in Section~\ref{subsubsec-logical-channel-interference}. We follow the same mark strategy as well. Specifically, we mark $x$ as \emph{linear}, $x^2$ as \emph{quadratic1}, $1-(x-1)^2$ as \emph{quadratic2}, $x^4$ as \emph{quartic1}, and $1-(x-1)^4$ as \emph{quartic2}. For each polynomial function, its SF is from 7 to 12. Hence, total 30 logical channels and corresponding SIR threshold heatmap (shown in Figure~\ref{fig-SIRheatmap}) are taken as the inputs for optimal channel selection Algorithm~\ref{alg-ChirpOptionAlgorithm}. We will study the impact of different maximum SIR threshold $SIR_T$ in Section~\ref{sec-SIR} to determine \ours configuration candidate set.


==> CurvingLoRa NSDI 22/6Implementation.tex <==
\section{Implementation}
\label{sec-implementation}

\vspace{1mm}
\noindent
\textbf{Hardware and software}. We implement \ours on software defined radios USRP N210 equipped with a UBX daughter board.
The modulation and demodulation are implemented based on UHD+GNURadio~\cite{url:gnu-radio}.
The transmitter and receiver work on the 904.0MHz ISM band, equipped with a VERT900 antenna~\cite{VERT900}. 
% and evaluate its performance on the software defined radios (SDRs), in which UHD+GNURadio \cite{url:gnu-radio} platform is aopted to launch \ours modulators/demodulators and monitor the carrier spectrum by real-time Short Time Fourier Transform (STFT). 
% The prototype of \ours is composed of a USRP N210~\cite{usrpn210} along with a UBX daughter board, operating at the 904.0MHz ISM band. 
% All radios are equipped with an VERT900 antenna~\cite{VERT900} to enhance below-GHz ISM band signal transmissions and receptions.
% Modulation and demodulation algorithms are achieved offline in Matlab and hardware-independent to be implemented on any commercial LoRa gateways as long as the physical samples can be obtained. 
By default, the spreading factor (SF) and bandwidth (BW) are set to 10 and 125 kHz, respectively.
The sampling rate is 1 MHz.


\begin{figure}
    \centering
    \includegraphics[width=0.37\textwidth]{figs/indoor.png}
    % \vspace{-4mm}
    \caption{The indoor experimental plan and SDR devices spread out across tens of rooms.}
    \label{fig-indoor-environment}
    \vspace{-4mm}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figs/outdoor.png}
    \vspace{-4mm}
    \caption{Bird view of the outdoor experiment field with the mobile gateway and LoRa nodes.}
    \label{fig-outdoor-environment}
    \vspace{-4mm}
\end{figure}

\begin{figure}[t]
\centering
\subfigure[Overall SER performance]{
    \includegraphics[width=0.495\columnwidth]{nsdi_figs_169/indoor_snr2ser_SF7911.pdf}
    \label{subfig-noise-resilience-no-collisions-1}
}\hspace{-0.06\columnwidth}
\subfigure[SER distribution in code space]{
	\includegraphics[width=0.495\columnwidth]{nsdi_figs_169/indoor_code2ser_.pdf}
    \label{subfig-noise-resilience-no-collisions-2}
}
% \vspace{-4mm}
\caption{Noise resilience in the absence of collisions.}
\label{fig-noise-resilience-no-collisions}
\vspace{-4mm}
\end{figure}

\begin{figure*}[t]
    \centering
    \subfigure[SER vs. SNR when SF=8]{
    \includegraphics[width=0.545\columnwidth]{nsdi_figs_169/snr2ser_symbol_SF8.pdf}
    \label{subfig-snr-in-collisions-symbol-1}
    }
    \hspace{-0.08\columnwidth}
      \subfigure[SER vs. SNR when SF=10]{
    \includegraphics[width=0.545\columnwidth]{nsdi_figs_169/snr2ser_symbol_SF10.pdf}
    \label{subfig-snr-in-collisions-symbol-2}
    }
    \hspace{-0.08\columnwidth}
    \subfigure[SER vs. SNR when SF=12]{
    \includegraphics[width=0.545\columnwidth]{nsdi_figs_169/snr2ser_symbol_SF12.pdf}
    \label{subfig-snr-in-collisions-symbol-3}
    }
    \hspace{-0.08\columnwidth}
    \subfigure[SER vs. symbol offset]{
    \includegraphics[width=0.545\columnwidth]{nsdi_figs_169/snr2ser_symbol_offset.pdf}
    \label{subfig-snr-in-collisions-symbol-4}	
    }
    % \vspace{-4mm}
\caption{Linear vs non-linear: symbol error rate ($SIR \approx 0dB$) in different spreading factor, SNRs and symbol offsets settings.}
\label{fig-snr-in-collisions-symbol}
% \vspace{-4mm}
\end{figure*}


\vspace{1mm}
\noindent
\textbf{Experiment setups}.
Due to LoRaWAN's constraint on channel access time (<1\% duty cycle ratio for each end node)~\cite{gamage_lmac_2020}, we conduct trace-driven emulations to evaluate our system. Specifically, we fix the gateway's location and move a transmitter to different sites. In each site, the transmitter sends packets in different spreading factors and chirp symbol settings.
We then align LoRa traces collected from different sites with varying symbol offset offline to emulate packet collisions.
The LoRa traces are collected in two different environments:

\noindent \textbf{$\bullet$} \textbf{Indoor scenario}. We place transmitters and gateway on a 30.48m$\times$21.34m office building. The offices are separated by concrete walls. Figure~\ref{fig-indoor-environment} shows the floor-plan of this office building. We place the gateway in the kitchen and move the transmitter to 10 different locations.
Due to the blockage of walls, most LoRa transmissions are under the non-line-of-sight (NLoS) condition.
    
\noindent \textbf{$\bullet$} \textbf{Outdoor scenario}. We deploy a campus-scale testbed outdoors.
The gateway powered by a UPS is placed on the parking lot. We move a transmitter to 12 locations and collect LoRa transmissions in both LoS and NLoS conditions with various link distances. The bird view of the outdoor testbed is shown in Figure~\ref{fig-outdoor-environment}. 
% The longest transmission distance between the USRP radio and the gateway is about 1,200m.


%the environment is the 3rd floor of an office building, covering 30.48m $\times$ 21.43m area with around 40 rooms, 

%We deploy the one USRP in the kitchen as the gateway (e.g., red point) and move our USRP radio in 10 positions (e.g., pink point), both are powered by a UPS battery. 
% For each position, we collect the LoRa packets under different SFs, types of chirp symbols (e.g., linear and non-linear) in multiple times. Due to the blockage of walls, most transmissions are under the non-line-of-sight (NLoS).

% For outdoor deployment, we deploy our test-bed at a campus-scale environment, in which the gateway is set at a parking lot and the USRP radio on the car is moved to 12 positions to collect LoRa transmissions under LoS and NLoS.
% The topology of the outdoor deployment is illustrated in Figure~\ref{fig-outdoor-environment}. 
% The longest transmission distance between the USRP radio and the gateway is about 1,200m.



\vspace{1mm}
\noindent
\textbf{Large-scale packet collision emulation}. Due to the temporal diversity (e.g., the cars passing by may block the LoS path or generate a new reflection path), the LoRa traces collected from each site experience significantly different channel variations. This allows us to emulate large-scale LoRa networks by reusing each individual LoRa trace as a transmission from a new LoRa transmitter.
We further enhance the link diversity by varying the SIR of each trace at the gateway. The symbol offset is randomly chosen from [0.2, 0.8]$\times$$T_{symbol\_time}$.
% To emulate different near-far issue, we take two approaches: $i)$: varying the transmission power, and $ii)$: adding white Gaussian noise to the received packet.

% also emulate large-scale collisions by manipulating the LoRa traces collected both indoors and outdoors.
% Specifically, we add different amount of white Gaussian noise to 


% we superimpose the LoRa packets transmit from different locations with random delays.
% Accordingly, packets collide with each other with different time offsets.
% To emulate different near-far issue, we take two approaches: $i)$: varying the transmission power, and $ii)$: adding white Gaussian noise to the received packet. 


%suppose packets from various positions with a configurable processing delay (smaller than a packet duration), delivering collided packets with different misalignment. 
%Hence, packets from transmitters collide at different parts with different time offsets (e.g., preambles, sync words, SFDs and payloads). 
%For fine- grained SNR and SIR control, we add white Gaussian noise with controlled amplitudes to the collected I and Q traces of packets and vary the transmitting power of the received packets to generate collisions under different near-far energy effects.

\vspace{1mm}
\noindent
\textbf{Evaluation Metrics}. We adopt three metrics to evaluate \ours. $i)$: \textit{Symbol Error Rate (SER)} measures the demodulation of \ours at the symbol level, under various SNRs and SIRs~\cite{tong_combating_2020,colora}; $ii)$: \textit{Packet Delivery Rate (PDR)} computes the packet reception rate. in which 80\% of symbols can be decoded successfully.\footnote {Most error correction codes can recover 1/5 symbol errors~\cite{tse2005fundamentals}.} $iii)$:  \textit{Throughput} can be derived with the received packets and decoded symbols, denoted by Symbol/Second. 
Note that LoRa gateways are usually deployed with tethered power supplies, and thus we do not consider energy consumption at the gateway~\cite{colora,tong_combating_2020}. 

\vspace{1mm}
\noindent
\textbf{Baselines}. We compare our design with two SOTA LoRa collision decoding systems, namely, successive interference cancellation-based mLoRa~\cite{mLoRa} and spectral energy-based NScale~\cite{tong_combating_2020}.
The standard LoRaWAN is also adopted as the baseline.
As a proof of concept, we design four types of non-linear chirps to evaluate: 
%$i)$: $quadratic1$---$f(t) = t^2$, $ii)$: $quadratic2$---$f(t) = -t^2+2t$, $iii)$: $quartic1$---$f(t) = t^4$, and $iv)$: $quartic2$---$f(t) = -t^4+4t^3-6t^2+4t$.
\vspace{-0.15in}
\begin{table}[h]
\small
\centering
\begin{adjustbox}{width=1\columnwidth}
\begin{tabular}{ll}
\hline 
 (1): $quadratic1$---$f(t) = t^2$ & (2): $quadratic2$---$f(t) = -t^2+2t$ \\
%\hline 
 (3): $quartic1$---$f(t) = t^4$ & (4): $quartic2$---$f(t) = -t^4+4t^3-6t^2+4t$ \\
\hline 
\end{tabular}
\end{adjustbox}
\vspace{-0.15in}
\end{table}




==> CurvingLoRa NSDI 22/7Evaluation.tex <==

\begin{figure*}[t]
    \centering
    \subfigure[SER vs. SIR when SF=8]{
    \includegraphics[width=0.535\columnwidth]{nsdi_figs_169/basic_sir2ser_symbol_SF8.pdf}
    \label{subfig-sir-in-collisions-symbol-1}
    }
    \hspace{-0.06\columnwidth}
    \subfigure[SER vs. SIR when SF=10]{
    \includegraphics[width=0.535\columnwidth]{nsdi_figs_169/basic_sir2ser_symbol_SF10.pdf}
    \label{subfig-sir-in-collisions-symbol-2}	
    }
    \hspace{-0.06\columnwidth}
    \subfigure[SER vs. SIR when SF=12]{
    \includegraphics[width=0.535\columnwidth]{nsdi_figs_169/basic_sir2ser_symbol_SF12.pdf}
    \label{subfig-sir-in-collisions-symbol-3}	
    }
    \hspace{-0.08\columnwidth}
    \subfigure[SER vs. symbol offset]{
    \includegraphics[width=0.535\columnwidth]{nsdi_figs_169/basic_offset2ser_symbol.pdf}
    \label{subfig-sir-in-collisions-symbol-4}	
    }
    % \vspace{-4mm}
    \caption{Linear vs. non-linear: symbol error rate ($SNR>30dB$) in different spreading factor, SIR, and symbol offset settings.}
    \label{fig-sir-in-collisions-symbol}
    % \vspace{-4mm}
\end{figure*}

\section{Evaluation}
\label{sec-evaluation}

We present the experiment results in this section. \S\ref{subsec-evaluation-1} first gives an overall comparison of \ours with linear chirps at the symbol and packet level, followed by the outdoor experiments at the campus scale in \S\ref{subsec-evaluation-2}. Finally, we provide the large-scale emulation to explore the impact of concurrency on \ours in \S\ref{subsec-evaluation-3}. And indoor evaluations can be found in $\S$\ref{appendix-3}.

% In this section, we first examine the noise resilience of \ours in controlled noises and symbol offset settings. 
% For fine-grained SNR control, we add white Gaussian noise with controlled amplitudes to the collected I and Q traces~\cite{tong_combating_2020,colora}.
% We then examine the symbol and packet error rate in different SIR conditions.
% We next evaluate the concurrent LoRa transmissions both indoors and outdoors.
% Finally, based on the collected data, we conduct emulations to explore the maximum concurrency of non-linear chirps.



\subsection{Overall Comparisons with Linear Chirps}\label{subsec-evaluation-1}

\vspace{1mm}
\noindent
\textbf{Noise resilience}. We first compare the noise resilience of \ours with linear chirps in the absence of collisions.
% Based on collected packets in our indoor test-bed, we manually add Gaussian noise and measure the SER. 
The results are shown in Figure~\ref{subfig-noise-resilience-no-collisions-1}.
In accordance with our analysis (\S\ref{subsec-design-3}), we observe that all four types of non-linear chirps in \ours demonstrate comparable noise resilience with linear chirps across all three $SF$ settings.
Figure~\ref{subfig-noise-resilience-no-collisions-2} shows that the symbol error rate is distributed evenly over the entire code space, confirming that the non-linear chirp achieves consistent SER for different symbols.
%Since Equation~\eqref{equ-shifted-nonlinear-chirps} encodes data uniformly on the frequency bins of non-linear chirps.

We also compare the noise resilience of \ours with LoRaWAN in the presence of collisions.
Figure~\ref{fig-snr-in-collisions-symbol}(a)-(c) shows the SER in various SNR and spreading factor settings.
When $SF$=8, we observe that both LoRaWAN and four types of non-linear chirps fail to demodulate packets in extremely low SNR conditions (i.e., SNR$\leq$-25$dB$).
As the SNR grows to $-15dB$, the SER achieved by non-linear chirps drops dramatically to around 1\%, whereas the SER of linear chirps is still above 20\%. As the SNR grows further, we observe the SER of non-linear chirps is always 10$\times$ lower than that of the linear chirps, e.g., 0.3\% versus 3\% at SNR=30$dB$.
Similar trends hold for $SF$=10 and 12.

\vspace{1mm}
\noindent
\textbf{Symbol offset}. Next, we compare the SER of \ours and linear chirps in various symbol offset settings.
Specifically, from our collected dataset, we randomly pick up LoRa symbols with different spreading factors (SF=8,10,12) and SNRs ([$-15dB$,$15dB$]). We then vary the symbol offset between two collision symbols from 10\% to 50\% and plot their SER in Figure~\ref{fig-snr-in-collisions-symbol}(d).
In consistency with our simulation in Figure~\ref{fig-nonlinear-vs-linear-tgap}, we observe the SER of linear chirps drops with increasing symbol offsets.
In contrast, the SER achieved by non-linear chirps maintains a consistent low level, with the maximal value of 1\% when the offset of two collision symbols is merely 10\%. In contrast, the SER achieved by linear chirps spans varies from 1\% to 80\% as the symbol offset decreases.
These results demonstrate that the non-linear chirps are robust to collisions with different symbol offsets.

% In case of collisions, we first evaluate the weak signal decoding at the symbol level, in which the weak target symbol collides with the two strong interfered symbols with a controlled symbol offset. Figure~\ref{fig-snr-in-collisions-symbol} shows the SER for \ours under different levels of SNRs with different SFs and symbol offsets.
% \ours can decode the collided weak symbol even with an extremely low SNRs as the non-linear chirps spread out the spectral energy of interfered chirp symbols and retains the inherent noise resilience of chirps. 
% For example, the SER keep under 1\% for \ours when $SNR>-15dB, -25dB, -25dB$ for $SF=8,10,12$, respectively.
% However, the performance gradually degrades for linear chirps under low SNR scenarios (e.g., $SNR<0dB$) in Figure~\ref{subfig-snr-in-collisions-symbol-1} to~\ref{subfig-snr-in-collisions-symbol-3}.
% In practice, small SFs in LoRa are adopted for near-range transmission with a high data rate, which can be adapted for the scenario of low SNRs to improve the decoding performance to a very low SER of 1\%~\cite{tong_combating_2020}.
% We also explore the impact of symbol time offsets, which lead to the packet misalignment in collisions. It has been shown that most recent studies~\cite{colora,tong_combating_2020,xia2019ftrack} rely on the time offset information to separate collided packets. 
% Figure~\ref{subfig-snr-in-collisions-symbol-4} shows the averaged SER of \ours in terms of the symbol time offsets, against the linear chirps. 
% The SER of linear chirps increases as packets collide with a smaller symbol time offset. Since a small offset induces a stronger spectral energy peak for interfered chirp symbols, consistent with our illustrations in Figure~\ref{fig-nonlinear-vs-linear-tgap}. While \ours performs reliably regarding various degrees of misalignment, with an average SER under 1\%.
% In practice, LoRa radios transmit packets in random time, where the symbol offset follows a uniform distribution within a symbol duration~\cite{tong_combating_2020}. 
% And \ours is agnostic to the offset variance in the real-life LoRa networks.

% We further compare \ours with the SIC-based mLoRa~\cite{mLoRa} at the packet level, from the preamble detection, packet alignment to the symbol decoding.
% Figure~\ref{fig-in-collisions-packet-1} illustrates \ours's superior performance under different SNRs, achieving an average SER less than 1\% when SNR>-20dB for all four types of non-linear chirps. In contrast, mLoRa only delivers an acceptable performance about $SNR=5dB$, which is determined by the inherent linear chirps and consistent with their experimental results~\cite{mLoRa,tong_combating_2020}.


\vspace{1mm}
\noindent
\textbf{Resolving near-far issue}.
We also compare \ours with linear chirp-based LoRa (i.e., LoRaWAN) in the presence of the near-far issue. 
In particular, we vary the SIR of the targeting symbol and measure its SER in each SIR setting.
Figure~\ref{fig-sir-in-collisions-symbol}(a)-(c) show the results in three different spreading factor settings.
We observe the standard LoRaWAN fails to decode weak targeting signal (i.e., SIR<$0dB$) across all three $SF$ settings.
In contrast, by leveraging the power scattering effect, all four types of non-linear chirps in \ours can successively demodulate weak symbols in the presence of strong collisions.
For instance, the averaging SIR threshold for achieving less than 1\% SER is -$3.7dB$, $-7.7dB$, and $-10.2dB$ for SF=8, 10, and 12, respectively.
We further vary the symbol offset of two collision symbols and measure the SER achieved by both \ours and LoRaWAN. The SIR and SF of symbols for evaluation varies from -$10dB$ to $1dB$, and from 8 to 12, respectively.
The results are shown in Figure~\ref{subfig-sir-in-collisions-symbol-4}.
We observe \ours achieves a robust low SER (i.e., less than 1\%) in the presence of a large symbol offset. It then degrades slightly as the symbol offset decreases. In contrast, the linear chirp achieves consistently high SER (i.e., $\geq$38\%) in all five different symbol offset settings.
%We attribute this to the side-lobe of the interfered chirp symbol when nearing the target one.
These results clearly demonstrate that \ours can successfully decode weak signals in the presence of strong collisions in various conditions.

% Figure~\ref{subfig-sir-in-collisions-symbol-1} to~\ref{subfig-sir-in-collisions-symbol-3} first show the SER for linear and non-linear chirps regarding SFs and SIRs, at the symbol level.
% LoRaWAN cannot decode the weak target signal (e.g., $SIR<0dB$) even if it is aligned and focuses the spectral energy of linear chirps.
% However, \ours harvests significant SIR gains by spreading the spectral energy of interfered chirp symbols. And it achieves the average SIR threshold of -3.7dB, -7.7dB, and -10.2dB for SF=8, 10, 12, above which the SER is less than 1\%. 

%Given the the uniform distribution of a symbol duration for packet misalignment in the real-life LoRa networking, \ours can successfully separate collisions in most cases. And we can further solve the decoding failures by using the re-transmission mechanism of LoRaWAN protocol.


% Figure~\ref{subfig-sir-in-collisions-symbol-4} further illustrates the relationship between the average SER and symbol offset across SIRs and SFs.
% In comparison with linear chirps, \ours first delivers robust SER less than 1\% with a larger symbol offset than 10\% while degrading slightly for a smaller offset. We attribute this to the side-lobe of the interfered chirp symbol when nearing the target one.
% Given the the uniform distribution of a symbol duration for packet misalignment in the real-life LoRa networking, \ours can successfully separate collisions in most cases. And we can further solve the decoding failures by using the re-transmission mechanism of LoRaWAN protocol.

\begin{figure}[t]
\centering
\subfigure{
    \includegraphics[width=0.48\columnwidth]{nsdi_figs_169/snr2ser_packet_10.pdf}
    \label{fig-in-collisions-packet-1}
}\hspace{-0.02\columnwidth}
\subfigure{
	\includegraphics[width=0.48\columnwidth]{nsdi_figs_169/sir2ser_packet_SF10.pdf}
    \label{fig-in-collisions-packet-2}
}
% \vspace{-4mm}
\caption{Head-to-head comparison with mLoRa\cite{mLoRa}.}
\label{fig-in-collisions-packet}
\vspace{-4mm}
\end{figure}

\begin{figure*}[t]
    \centering
    \subfigure{
    \includegraphics[width=0.68\columnwidth]{nsdi_figs_169/outdoor_ser_10.pdf}
    \label{subfig-outdoor-1}
    }
    \hspace{-0.06\columnwidth}
    \subfigure{
    \includegraphics[width=0.68\columnwidth]{nsdi_figs_169/outdoor_pdr_10.pdf}
    \label{subfig-outdoor-2}	
    }
    \hspace{-0.06\columnwidth}
    \subfigure{
    \includegraphics[width=0.68\columnwidth]{nsdi_figs_169/outdoor_throughput_10.pdf}
    \label{subfig-outdoor-3}	
    }
    % \vspace{-4mm}
    \caption{Outdoor experiment: examine the impact of concurrent transmissions on SER, PDR, and network throughput.}
    \label{fig-outdoor}
     \vspace{-4mm}
\end{figure*}

\vspace{1mm}
\noindent
\textbf{Head-to-head comparison with mLoRa\cite{mLoRa}}. We compare \ours with mLoRa on using our indoor dataset.
Figure~\ref{fig-in-collisions-packet-1} shows the SER of each system in the presence of two collision packets.
We observe that the SER of mLoRa drops gradually from 15\% to 1\% as the SNR grows from -$15dB$ to 15$dB$.
It finally drops to 0.3\% when SNR grows to $30dB$.
In contrast, all four types of non-linear chirps adopted by \ours achieve a consistently low SER ($\leq$0.01\%) when SNR is larger than -$15dB$.
Similarly, as shown in  Figure~\ref{fig-in-collisions-packet-2}, the SER of mLoRa is over 10\% in the presence of a strong collision (i.e., $SIR<0dB$) whereas \ours can demodulate weak signals at an $SER<1\%$ as long as the SIR is larger than -$12dB$.


% In the basic two-packet collisions from the indoor test-bed, we further evaluate the performance for \ours and mLoRa~\cite{mLoRa} in the whole packet processing. 
% Figure~\ref{fig-in-collisions-packet-2} shows that mLoRa~\cite{mLoRa} performs consistently with an average SER larger than 30\%.
% In contrast, \ours delivers excellent SIR tolerance for decoding weak signals in collisions, achieving an average SER under 1\% when SIR is larger than -14dB for all four types of non-linear chirps.
% Evaluations also demonstrate the effectiveness of our strategies on packet detection and alignments ($\S$\ref{subsec-system-3}), which guarantees the performance of \ours on non-linear payload decoding.
 

\vspace{1mm}
\noindent
\textbf{Remarks}. These experiments show the advantage of \ours in dealing with near-far issues. It also reveals that the performance of \ours varies with the non-linear function being adopted.
Overall the quadratic function $f(t) = t^2$ achieves consistently better SER than the other types of non-linear functions. 
We leave the exploration of non-linear space as our future work.


% \subsection{Concurrency in the Indoor Environment}
% \begin{figure*}[t]
%     \centering
%     \subfigure{
%     \includegraphics[width=0.68\columnwidth]{nsdi_figs_169/indoor_ser_10.pdf}
%     \label{subfig-indoor-1}
%     }
%     \hspace{-0.06\columnwidth}
%     \subfigure{
%     \includegraphics[width=0.68\columnwidth]{nsdi_figs_169/indoor_pdr_10.pdf}
%     \label{subfig-indoor-2}	
%     }
%     \hspace{-0.06\columnwidth}
%     \subfigure{
%     \includegraphics[width=0.68\columnwidth]{nsdi_figs_169/indoor_throughput_10.pdf}
%     \label{subfig-indoor-3}	
%     }
%     \vspace{-4mm}
%     \caption{Indoor experiment: examine the impact of concurrent transmissions on SER, PDR, and network throughput.}
%     \label{fig-indoor}
%     \vspace{-4mm}
% \end{figure*}

% We then examine the scalability of \ours on decoding collisions in various numbers of concurrent transmissions (termed as $N$).
% In particular, we measure the SER, packet delivery rate, and network throughput and compare it with  mLoRa~\cite{mLoRa}, NScale~\cite{tong_combating_2020}, and LoRaWAN three baselines.


% As $N$ grows from 2 to 10, the SER of LoRaWAN, mLoRa, and NScale all increases gradually, as shown in Figure~\ref{subfig-indoor-1}.
% Specifically, LoRaWAN can only demodulate the strongest transmission in all different of $N$ settings. 
% mLoRa, on the other hand, 
% achieves better performance than LoRaWAN. It however still achieves a high SER (i.e., $\geq$40\%) when more than three transmitters work concurrently.
% NScale performs better than above two schemes, with a SER grows gradually from less than 10\% to 40\% as $N$ grows to 10 due to the severe near-far issue. 
% In contrast, \ours achieves an average SER of less than 10\% in all different $N$ settings.

% Figure~\ref{subfig-indoor-2} shows the packet delivery ratio achieved by these systems. We observe that as $N$ grows, the PDR achieved by \ours drops slightly from 100\% to 85\%.
% In contrast, the PDR drops significantly to less than 60\%, 40\%, and 10\% for NScale, mLoRa, and LoRaWAN, respectively.
% We further compute the network throughput and plot the results in Figure~\ref{subfig-indoor-3}.
% The overall network throughput of \ours, NScale, and mLoRa all grows with increasing $N$.
% The network throughput of LoRaWAN, manifests a converse trend due to the magnified interference as $N$ grows.
% Taking a further scrutiny on this results, we find that the network throughput of \ours grows almost linearly with $N$.
% In contrast, the growing trend of network throughput in both NScale and mLoRa drops gradually as $N$ grows. This is because the near-far issue grows extensively with increasing number of concurrent transmissions. However, both NScale and mLoRa are not scale to such circumstances.
% %However, mLoRa and NScale grows up much more slowly than \ours. Since both of them cannot account for the near-far effect well.
% %While \ours's throughput increases almost linearly, nearing the ideal one as the increment of concurrency.
% Statistically, when $N$=10, the overall network throughput of \ours is 6.58$\times$, 2.63$\times$, and 1.63$\times$ higher than that of LoRaWAN, mLoRa, and NScale, respectively.


\subsection{Concurrency at the Campus Scale}\label{subsec-evaluation-2}

We evaluate \ours on decoding collisions in different numbers of concurrent transmissions (termed as $N$) settings.
In particular, we measure the SER, PDR, and network throughput and compare with mLoRa~\cite{mLoRa}, NScale~\cite{tong_combating_2020}, and LoRaWAN three baselines. We repeat the experiments in indoor environments and put the results in Appendix \ref{appendix-3}.

%We repeat above experiments in outdoor environment where the link distance is significantly longer. The SIR of the received signal varies from $-15dB$ to $-3dB$ under low SNR conditions. 
%We superpose the collected packets from 12 different locations and evaluate \ours’s performance in different settings.

% Figure~\ref{fig-outdoor} shows the SER, PDR, and network throughput of the standard LoRaWAN, mLoRa, and \ours in different number of concurrent transmissions. 

As $N$ grows, the SER of LoRaWAN, mLoRa, and NScale all increase gradually, as shown in Figure~\ref{subfig-outdoor-1}.
Specifically, LoRaWAN can only demodulate the strongest transmission for most settings.
And mLoRa achieves a slightly better performance than LoRaWAN. However, its SER aggravates significantly ($\geq$50\%) when demodulating more than four concurrent transmissions. Besides, NScale performs better than the above two schemes, and the SER grows gradually from less than 15\% to 55\% when $N$ grows to 12.
In contrast, \ours achieves an average SER of less than 25\% in all settings.

Figure~\ref{subfig-outdoor-2} shows the packet delivery ratio achieved by these systems. We observe that as $N$ grows, the PDR achieved by \ours drops slightly from 100\% to 65\%.
In contrast, the PDR drops significantly to less than 36.5\%, 25.0\%, and 12.5\% for NScale, mLoRa, and LoRaWAN, respectively.
We further compute the network throughput and plot the results in Figure~\ref{subfig-outdoor-3}.
The overall network throughput of \ours, NScale, and mLoRa grow with the increasing $N$.
However, the network throughput of LoRaWAN manifests a converse trend due to the magnified interference as $N$ grows.
Taking a further scrutiny on this result, we find that the network throughput of \ours grows almost linearly with $N$.
In contrast, the growing trend of network throughput in both NScale and mLoRa drops gradually as $N$ grows. This is because the near-far issue grows extensively with an increasing number of concurrent transmissions. However, both NScale and mLoRa are not scaling to such circumstances. Statistically, when $N$=12, the average network throughput of \ours is 5.21$\times$, 2.61$\times$, and 1.84$\times$ higher than that of LoRaWAN, mLoRa, and NScale, respectively.

% {
% \textcolor{blue}{
% Similar to the SER trend of indoor experiments, we observe a huge SER gap between \ours and its competitors as $N$ grows in outdoor experiments (Figure~\ref{subfig-outdoor-1}).
% On the other hand, compared with indoor experiments, we find that all systems in outdoor spaces achieve slightly higher SER.
% This is because the transmitters are facing much severe near-far issue outdoors.
% The packet delivery rate in outdoor experiments also shows the similar trend with their indoor counterparts, as shown in Figure~\ref{subfig-outdoor-2}. Specifically, the PDR achieved by \ours drops slightly from 100\% to 80\% on average as $N$ grows from 2 to 12.
% While both mLoRa and LoRaWAN drops significantly from around 50\% to less than 40\% and 10\%, respectively.
% Figure~\ref{subfig-outdoor-3} shows the network throughput achieved by these three systems in outdoor environment.
% The overall network throughput of \ours grows up consistently as the number of transmitters scales up. When 10 packets collide simultaneously with significant power difference, the network throughput of \ours in average is about 2.8$\sim$7.6$\times$ higher than the network throughput achieved by mLoRa and the standard LoRaWAN.
% On the other hand, we observe that the PDR and network throughput achieved by \ours both suffers as $N$ grows further to 12.
% We thus investigate this result and find this is due to the sharp drop of SIR as $N$ grows to 12.}}

% \subsection{Exploring the Maximal Concurrency}
% \begin{figure}[t]
%     \centering
%     \subfigure[SIR$\in$[-5dB, 0)]{
%     \includegraphics[width=0.49\columnwidth]{figs/indoor_packet_largescale_sir5_10.png}
%     \label{subfig-maximum-1}
%     }
%     \hspace{-0.06\columnwidth}
%     \subfigure[SIR$\in$[-10dB, 0)]{
%     \includegraphics[width=0.49\columnwidth]{figs/indoor_packet_largescale_10.png}
%     \label{subfig-maximum-2}	
%     }
%     \caption{Emulation of weak signal decoding over large-scale collisions}
%     \label{fig-maximum}
% \end{figure}

\subsection{Large-scale emulation}\label{subsec-evaluation-3} 
We also emulate large-scale collisions using the data collected both indoors and outdoors.
Specifically, in each number of concurrent transmission settings, we only measure the SER of the weakest transmissions as those stronger transmissions are likely to be correctly demodulated.
Figure~\ref{subfig-maximum-1} shows the SER of \ours and LoRaWAN when the SIR varies randomly between [$-5dB$,$0dB$], We observe that all four types of non-linear chirps adopted by \ours can successively demodulate the weakest transmission (i.e., SER=0) when the number of concurrent transmissions is less than 30. The SER then grows up gradually as the network scales.
It peaks at 50\% when 100 transmitters work concurrently.
In contrast, the standard LoRaWAN fails to demodulate the weakest transmission when there are more than two concurrent transmissions.
%slowly as the network scales up and reaches 50\% in collisions of 100 packets.
%The performance of \ours suffers with the intensified near-far effect, 
% Figure~\ref{subfig-maximum-2} illustrates the 50\% SER of \ours when 50 packets collide, whose SIR varies from $-10dB$ to 0.


% TBD
% \subsection{TBD: Non-linear Chirp Candidates}
% \begin{figure}[t]
%     \centering
%     \subfigure[SF=10]{
%     \includegraphics[width=0.49\columnwidth]{figs/sir2map_fs125k_SF10_bar_sine_part.png}
%     \label{subfig-inter-sf-1}	
%     }
%     \hspace{-0.06\columnwidth}
%     \subfigure[SF=12]{
%     \includegraphics[width=0.49\columnwidth]{figs/sir2map_fs125k_SF12_bar_sine_part.png}
%     \label{subfig-inter-sf-2}	
%     }
%     \caption{SIR Threshold for co-SF and inter-SF collisions}
%     \label{fig-inter-sf}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{nsdi_figs_169/indoor_packet_largescale_sir5_10.pdf}
     \vspace{-4mm}
    \caption{Emulation of large-scale collisions.}
     \vspace{-4mm}
    \label{subfig-maximum-1}
\end{figure}

==> CurvingLoRa NSDI 22/8RelatedWork.tex <==
\section{Related Work}
\label{sec-related-work}

% LoRWAN researches
% In recent years, a variety of studies~\cite{dongare2018charm,peng2018plora,gadre2020frequency,IPSN2019, liu_deeplora_nodate, gamage_lmac_2020,LoSee,liando2019known} witness the rapid research progress in LoRaWANs.
% An important branch focuses on resolving collision issues~\cite{lora_survey_1}. 
% Meanwhile, the non-linear chirp signal has been utilized in communication and radar systems. 

Prior work on resolving LoRa collisions has followed a common theme: exploring the unique features of collided LoRa symbols in the time domain~\cite{mLoRa,oct,xia2019ftrack}, frequency domain~\cite{colora,tong_combating_2020,xu_fliplora_2020,eletreby2017empowering}, or both~\cite{hu2020sclora,shahid2021concurrent}.
For instance, mLoRa~\cite{mLoRa} observes that collisions usually start with a stretch of interference free bits on the packet header. The receiver can thus decode these uncontaminated bits first and then leverage successive interference cancellation~\cite{gollakota2009interference,mollanoori2013uplink} to decode the collided bits iteratively.
Choir~\cite{eletreby2017empowering} uses the frequency variation caused by oscillator imperfection to map bits to each individual LoRa transmitter.
FTrack~\cite{xia2019ftrack} jointly exploits the distinct tracks on the frequency domain and misaligned symbol edges in the time domain to separate collisions.
By combining spectra obtained from different parts within each symbol, CIC~\cite{shahid2021concurrent} exploits the sub-symbols that provide both time and frequency resolution to cancel out the interference under low SNR conditions (\emph{e.g.}, above $-10$~dB).

While above ideas have demonstrated their efficacy, they still face two scalability issues that fundamentally challenge their applicability in practice:
First, the vast majority of these approaches do not scale to a large number of concurrent transmissions. For instance, mLoRa~\cite{mLoRa} and FTrack~\cite{xia2019ftrack} barely support up to three concurrent transmissions to maintain a symbol error rate less than 0.1. While Choir~\cite{eletreby2017empowering} improved over the above methods, it does not scale to more than ten devices. Although NScale~\cite{tong_combating_2020} can support tens of concurrent transmissions, it requires the overlap ratio between different symbols to be lower than a rigid threshold, which is unlikely to be held in practice given laissez-faire LoRa transmissions.
Second, none of the foregoing approaches scale well to near-far deployment scenarios. This is due to the fact that after dechirping, the weak reception from a remote transmitter produces a tiny FFT peak that is likely to be buried by strong FFT peaks from LoRa nodes that are closer to the receiver. 

Although successive interference cancellation (SIC) can be leveraged to deal with this near-far issue, it functions only in high SNR conditions due to the following reasons.
First, due to Carrier Frequency Offset (CFO) and Sampling Frequency Offset (SFO), the phase of received chirp symbols is likely to distort by a certain degree.
This phase distortion is critical to the success of signal recovery in SIC but is difficult to estimate in low SNR conditions~\cite{colora}.
Second, SIC suffers from hardware imperfections~\cite{tong_combating_2020}, which is common on low-end IoT devices. The symbol recovering error accumulates gradually and is likely to fail the SIC in the end. In addition, the impact of ambient RF noise on SIC, particularly the parameter estimation for signal reconstruction, gets exacerbated at low SNR conditions.
Instead of leveraging new features on time or frequency domain to combat LoRa collisions, \ours addresses this issue from a fresh new angle and designs LoRa signals to facilitate concurrent transmissions. 
%studies the case for non-linear chirp-based LoRa transmissions and demonstrate such design can effectively improve the parallel LoRa transmissions even in the extreme SNR and SIR conditions.

% \vspace{1mm}
% \noindent
% \textbf{Resolving lora collisions}. There are a bunch of works on resolving LoRa collisions. Choir~\cite{eletreby2017empowering} extracts the unique frequency drift introduced by LoRa radios to disentangle concurrent LoRa transmissions.
% mLoRa~\cite{mLoRa} proposes to leverage the temporal features to demodulate collision packets. 
% FTrack~\cite{xia2019ftrack} combines the frequency and temporal features to demodulate collisions.
% However, as we experimentally demonstrated, these systems do not scale well to low SNR conditions.
% CIC~\cite{shahid2021concurrent} outperforms LoRaWAN~\cite{alliance2020lorawan} and FTrack~\cite{xia2019ftrack} under low SNR conditions by using the fine-grained sub-symbols that provides both time and frequency resolution.
% CoLoRa~\cite{colora} and NScale~\cite{tong_combating_2020} translate the packet time offset into \textit{spectral peak ratio} to enable collision demodulation in low-SNR conditions.
% Different from these designs, \ours studies the case for non-linear chirp-based LoRa transmissions and demonstrate such design can effectively improve the parallel LoRa transmissions even in the extreme SNR and SIR conditions.

Nonlinear frequency modulation has been widely used in radar systems. Lesnik \emph{et al.} \cite{lesnik2008modification} demonstrate that using nonlinear frequency modulation can enhance signal sensitivity.
Doerry \emph{et al.} \cite{doerry2006generating} and Benson \emph{et al.} \cite{benson2015modern} details the way to build non-linear chirp receivers.
%Some works reported how non-linear chirp can benefit communication systems.
Kahn \emph{et al.} \cite{khan2013performance} and 
Hosseini \emph{et al.} \cite{hosseini2019nonlinear, hosseini2021nonlinear} use nonlinear chirps in Multi user orthogonal chirp spread spectrum (MU-OCSS) communication system to mitigate the multiple access interference problem.
Wang \emph{et al.} \cite{wang2015non} propose to use non-linear chirps for communication systems of binary orthogonal keying mode.
In contrast to these efforts, \ours explores a new possibility of using non-linear chirps to improve reception of concurrent LoRa-like signals.
%In comparison with these works, \ours focus on the possibility that utilize non-linear chirps to benefit the throughput of the wide-area IoT, a totally brand-new scenario. 
%which is totally different with radar systems and the modulation methods of the studied communication systems.
%\ours benefits from nonlinear chirps, then designs end-to-end modulation/ demodulation methods and logical channel selection algorithm to enhance LoRaWAN capacity.


==> CurvingLoRa NSDI 22/9Discussion.tex <==
%\section{Discussion}
%Here we outline three system opportunities of \ours to further exhibit its extensions over LoRa Design.
%
%1) \emph{Packet Wrapping}. Present design of \ours packets doesn't introduce coding rate(CR) configure in LoRa. This PHY-layer parameter can improve the robustness of delivered packets under the circumstance of bit error occurrence. Although \ours focuses on the modem design of chirp spread spectrum, methods like limiting packet length and setting different preamble upchirp count can reduce packet loss occurring on the demodulator side.
%
%2) \emph{Hardware Implementation}. Present prototype of HackRF and USRP is not a perfect implementation of \ours, as an extension to Semtech LoRa Chip. Although HackRF prototype proves the feasibility of \ours design, its dependence on Raspberry Pi can't reveal its potential low power feature. Also, evaluated by universal software defined radios, \ours doesn't have much power gain to show similar long-range coverage as LoRa SX1255 integration\cite{SX1255}, which is specially designed for narrow-band communication and embedded as the RF front end of LoRa gateways. Implementation with SX1255 and low-power stm32 can help build a large-scale \ours system.
%
%3) \emph{MAC-layer protocols}. The most popular MAC-layer protocol of LoRa is LoRaWAN, whose design is based on ALOHA access with limitation of 1\% duty cycle. In some scenarios involving near-far problems and multiple physical channel choices, time-slotted allocation will increase the network throughput and capacity. Such designs have been explored for LoRa systems\cite{hessar2018netscatter,liando2019known}. Since \ours configurations shares similar SNR and SIR sensitivity with LoRa, MAC-layer techniques can help enhance \ours performance.
